The Effectiveness of Strategies to Contain SARS-CoV-2: Testing, Vaccinations, and NPIs

In order to slow the spread of the CoViD-19 pandemic, governments around the world have enacted a wide set of policies limiting the transmission of the disease. Initially, these focused on non-pharmaceutical interventions; more recently, vaccinations and large-scale rapid testing have started to play a major role. The objective of this study is to explain the quantitative effects of these policies on determining the course of the pandemic, allowing for factors like seasonality or virus strains with different transmission profiles. To do so, the study develops an agent-based simulation model, which is estimated using data for the second and the third wave of the CoViD-19 pandemic in Germany. The paper finds that during a period where vaccination rates rose from 5% to 40%, large-scale rapid testing had the largest effect on reducing infection numbers. Frequent large-scale rapid testing should remain part of strategies to contain CoViD-19; it can substitute for many non-pharmaceutical interventions that come at a much larger cost to individuals, society, and the economy.

==> figures/results/tables/role_of_work_rapid_tests_table.tex <==
\begin{tabular}{lr}
\toprule
{} &  predicted total infections from 2021-01-01 until 2021-05-31 \\
scenario                  &                                                              \\
\midrule
 without work rapid tests &                                            2656668 \\
 baseline                 &                                            2303204 \\
\bottomrule
\end{tabular}


==> figures/results/tables/student_infections_table.tex <==
\begin{tabular}{lr}
\toprule
{} &  predicted total infections among 5-14 year olds from Easter until 2021-05-31 \\
scenario                               &                                                                               \\
\midrule
 educ open after easter  without tests &                                             725914 \\
 educ open after easter  with tests    &                                             552894 \\
 close educ after easter               &                                             430594 \\
 baseline                              &                                             439077 \\
\bottomrule
\end{tabular}


==> paper/results.tex <==
\section{Results}
\label{sec:results}

This is the results section.

\begin{figure}[ht]
  \centering
  \begin{subfigure}{.6\textwidth}
    \includegraphics[width=0.9 \textwidth]{figures/results/figures/scenario_comparisons/one_off_and_combined/full_new_known_case_cropped}
  \end{subfigure}%
  \begin{subfigure}{.6\textwidth}
    \includegraphics[width=0.9 \textwidth]{figures/results/figures/scenario_comparisons/one_off_and_combined/full_newly_infected_cropped}
  \end{subfigure}
  \caption{The Effect of Policies on Observed and Unobserved Cases}
  \label{fig:explain_decline}
  \figurenotes{\ldots}
\end{figure}

\begin{figure}[ht]
  \centering
  \begin{subfigure}{.6\textwidth}
    \includegraphics[width=0.9 \textwidth]{figures/results/figures/scenario_comparisons/school_scenarios/full_new_known_case}
  \end{subfigure}%
  \begin{subfigure}{.6\textwidth}
    \includegraphics[width=0.9 \textwidth]{figures/results/figures/scenario_comparisons/school_scenarios/full_newly_infected}
  \end{subfigure}
  \caption{The Effect of Different School Scenarios on Observed and Unobserved Cases}
  \figurenotes{}
  \label{fig:appdx_school_scenarios}
\end{figure}


\FloatBarrier

\input{figures/results/tables/student_infections_table}

\FloatBarrier


==> templates/Preamble_BibLaTeX_AER_Poster.tex <==
% !TeX program = pdflatex
% !TeX TXS-program:compile = txs:///pdflatex/
% !TeX TS-program = pdflatex
% !BIB program = biber
% !TeX TXS-program:bibliography = txs:///biber




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  CITATION COMMANDS AND BIBLIOGRAPHY STYLE %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% AER/JEL/JEP style

\usepackage[backend=biber, natbib=true, bibencoding=inputenc, bibstyle=authoryear, citestyle=authoryear-comp, mincitenames=1, maxcitenames=2, minbibnames=1, maxbibnames=7, uniquename=false, uniquelist=true, giveninits=true, backref=false, doi=false, url=false, isbn=false, dashed=false, sorting=ynt, sortcites=true, mergedate=true, dateabbrev=false, abbreviate=false, citetracker=true]{biblatex}
% sortcites sorts the in-text citations by year of publication
\DeclareBibliographyAlias{newspaper}{article}

%% Full author list on first citation, ``et al.'' only from second citation onwards:
%% https://tex.stackexchange.com/questions/48846/biblatex-et-al-beginning-from-second-citation
%% ==>
%%\AtEveryCitekey{\ifciteseen{}{\clearfield{namehash}}}  % Uncomment this ``so that an entry won't be part of a compact citation list the first time it is cited.''
%\xpatchbibmacro{cite}
%	{\printnames{labelname}}
%	{\ifciteseen
%		{\printnames{labelname}}
%		{\printnames[][1-5]{labelname}}%
%	}
%	{}
%	{}
%\xpatchbibmacro{textcite}
%	{\printnames{labelname}}
%	{\ifciteseen
%		{\printnames{labelname}}
%		{\printnames[][1-5]{labelname}}%
%	}
%	{}
%	{}
%% <==

\let\citeorig\cite
\renewcommand{\cite}{\citet}
\renewcommand{\citealp}{\citeorig}

\defbibheading{subbibliography}[\refname]{%
	\section*{#1}%
	\sectionmark{#1}%
	\addcontentsline{toc}{section}{#1}%
}

\renewcommand{\bibfont}{\sffamily\small}
	% Reduce font size for the bibliography, make the font sans-serif.
\setlength{\bibindent}{\parindent}
\setlength{\bibitemsep}{0pt}

\DefineBibliographyStrings{english}{%
	andothers = {et~al\adddot},
	volume = {vol\adddot}
}

% Remove parentheses from the date:
\xpatchbibmacro{date+extradate}{%
	\printtext[parens]%
}{%
	\setunit*{\mkbibbold{\addperiod\space}}%
	\mdseries\selectfont\printtext%
}{}{}
% Make the author/editor name(s) bold ==>
% See https://tex.stackexchange.com/questions/41468/biblatex-textcite-author-formatting-vs-bibliography-author-formatting
\xpatchbibmacro{author}{\printnames{author}}{\mkbibbold{\printnames{author}\addperiod}}{}{}
%\xpretobibmacro{author}{\mkbibbold\bgroup}{}{}
%\xapptobibmacro{author}{\egroup}{}{}
\xpretobibmacro{editor+others}{\mkbibbold\bgroup}{}{}%
\xapptobibmacro{editor+others}{\egroup\clearname{editor}}{}{}%
\xpretobibmacro{translator+others}{\mkbibbold\bgroup}{}{}%
\xapptobibmacro{translator+others}{\egroup\clearname{translator}}{}{}
% Set up page range compression (e.g., 1034-1067 => 1034-67)
\setcounter{mincomprange}{100}
\setcounter{maxcomprange}{100000}
\setcounter{mincompwidth}{10}
\DeclareFieldFormat{pages}{\mkcomprange{#1}}
% Removes ``pp.'' from pages and compresses page ranges:
\DeclareFieldFormat[article, inbook, incollection, inproceedings, patent, thesis, unpublished, newspaper]{pages}{{\nopp\mkcomprange{#1}}} 
% Include comma also after first name in the case of only two authors:
\AtEveryBibitem{
	\renewcommand*{\finalnamedelim}{\finalandcomma\addspace\bibstring{and}\space}
	\renewcommand*{\finallistdelim}{\finalandcomma\addspace\bibstring{and}\space}
}
\xpretobibmacro{byeditor+others}  % Undo this for the listing of editors
	{%
		\renewcommand*{\finalnamedelim}{%
			\ifnumgreater{\value{liststop}}{2}{\finalandcomma}{}%
			\addspace\bibstring{and}\space%
		}%
	}
	{}
	{\DoNotContinue}

% \renewcommand*{\newunitpunct}{\addcomma\space}
\renewcommand*{\bibnamedash}{---{\kern -2.25pt}---{\kern -2.25pt}---\addcomma\space}

%\DeclareCiteCommand{\citejournal}
%  {\usebibmacro{prenote}}
%  {\usebibmacro{citeindex}%
%   \usebibmacro{journal}}
%  {\multicitedelim}
%  {\usebibmacro{postnote}}

% Remove ``in'' for journal and newspaper articles:
\renewcommand*{\intitlepunct}{\space}
\renewbibmacro{in:}{%
	\ifentrytype{article}%
		{}%
		{\ifentrytype{newspaper}%
			{}%
			{\printtext{\bibstring{in}\intitlepunct}}%
		}%
}

% How to handle DOIs and URLs
% ==>
%\renewbibmacro*{doi+eprint+url}
%{%
%	\iffieldundef{doi}
%	{}
%	{\printfield{doi}}
%	\newunit\newblock
%	\iftoggle{bbx:eprint}
%	{\usebibmacro{eprint}}
%	{}%
%	\newunit\newblock
%	\iffieldundef{doi}  % If no DOI provided, use URL
%	{\usebibmacro{url+urldate}}
%	{}
%}
%% Remove URLs to save space
%\AtEveryBibitem{
%	\ifentrytype{article}%
%		{\clearfield{url}}% then
%		{}% else
%}
\DeclareFieldFormat{url}{%
	% \setlength{\Urlmuskip}{0mu}%
	\Urlmuskip = 0mu\relax%
	\caps{URL}\addcolon\space\url{#1}%
}
% Link DOIs automatically to https://doi.org/<DOI>:
\DeclareFieldFormat{doi}{%
	% \setlength{\Urlmuskip}{0pt}%
	\Urlmuskip = 0mu\relax
	\caps{DOI}\addcolon\space\href{https://doi.org/#1}{\nolinkurl{#1}}%
}
% <==

% Make journal title italic:
\DeclareFieldFormat[article]{journaltitle}{%
	\mkbibemph{#1}%
	\iffieldundef{volume}{\addcomma}{}%
}

% Handling of newspaper articles
\DeclareFieldFormat[newspaper]{journaltitle}{%
	\mkbibemph{#1} \mkbibparens{\thefield{edition}}\addcomma\addspace%
	\iflanguage{ngerman}{%
		\addnbspace\thefield{day}\addperiod\addnbspace\mkbibmonth{\thefield{month}}\addspace\thefield{year}%
	}{% else: default to the USenglish version
		\mkbibmonth{\thefield{month}}\addnbspace\thefield{day}\addcomma\addspace\thefield{year}%
	}%
	\iffieldundef{volume}{\addcolon}{\addcomma}%
}
\DeclareFieldFormat[newspaper]{date}{%
	\thefield{year}%
}

% Format the ``month'' field:
\DeclareFieldFormat{month}{\mkbibmonth{#1}}

% Put the title of articles in quotation marks:
\DeclareFieldFormat[thesis, unpublished, report, misc, newspaper]{title}{\mkbibquote{#1}}
%% Make title of books italic:
%\DeclareFieldFormat[book]{title}{\mkbibemph{#1}\nopunct}

% Makes first character of document type uppercase:
\DeclareFieldFormat[thesis, unpublished, report, misc]{type}{\MakeCapital{#1}}

%% Remove punctuation after ``series'' field:
%\DeclareFieldFormat[incollection]{series}{#1\nopunct}

% Add ``vol.'' for books etc.:
\DeclareFieldFormat[book, inbook, incollection, inproceedings]{volume}{\bibstring{volume}\addnbspace#1\addcomma}
% Formatting VV\,(NN):
\DeclareFieldFormat[article]{volume}{%
	\iffieldundef{volume}{}{%
		\addspace#1%
		\iffieldundef{number}{\addcolon}{\nopunct}%
	}
}
\DeclareFieldFormat[article]{number}{\addnbthinspace\mkbibparens{#1}\addcolon}
\DeclareFieldFormat[article]{date}{#1}

% \AtEveryCitekey{\clearfield{month}}
% Replace number by month if number is undefined:
% ==>
\DeclareSourcemap{
    \maps[datatype=bibtex]{
        \map{
            \pertype{article}
			\step[notfield=number, final]
			\step[fieldsource=month, fieldtarget=number]
            \step[fieldset=month, null]
            \step[fieldset=month_numeric, null]
        }
    }
}
% <==

% Adjust formatting of back-references
% ==>
\DefineBibliographyStrings{english}{%
	backrefpage  = {},	% originally ``cit. on p.''
	backrefpages = {}	% originally ``cit. on pp.''
}
\DefineBibliographyStrings{ngerman}{%
	backrefpage  = {},	% originally ``Siehe Seite''
	backrefpages = {}	% originally ``Siehe Seiten''
}
\renewcommand*{\finentrypunct}{}
\renewbibmacro*{pageref}{%
	\addperiod
	\iflistundef{pageref}
	{}
	{\printtext[brackets]{%
			\ifnumgreater{\value{pageref}}{1}
			{\bibstring{backrefpages}}
			{\bibstring{backrefpage}}%
			\printlist[pageref][-\value{listtotal}]{pageref}%
		}%
	}%
}
% <==

% Move notes to the end of an entry by copying the ``note'' information into ``addendum'': -->
\DeclareSourcemap{
	\maps[datatype=bibtex]{
		% Copy values of the Mendeley-created ``annote'' field to the ``note'' field:
		\map[overwrite]{
		 	\step[fieldsource=annote]
		 	\step[fieldset=note, origfieldval, append]
			\step[fieldset=annote, null]
		}
		\map{
			\step[fieldsource=note, final]
			\step[fieldset=addendum, origfieldval, final]
			\step[fieldset=note, null]
		}
	}
}
% \DeclareFieldFormat{addendum}{(#1)} % Enclose addendum/note in parentheses.
% <--

\AtEveryBibitem{%
	\ifentrytype{newspaper}%
		{\clearfield{addendum}}% then
		{\clearfield{month}}% else
}

% Add ``working paper'' as the default value for type of ``techreports'' ==>
% see https://tex.stackexchange.com/questions/212362/how-to-use-declaresourcemap-to-add-default-value-to-a-field
\DeclareSourcemap{
	\maps[datatype=bibtex]{
		\map{% Will overwrite fields without the ``overwrite'' option
			\pertype{techreport}
			\step[fieldset=type, fieldvalue={Working paper}]
		}
	}
}
% <==

% Add “doctoral dissertation” as the default value for type of “phdthesis” ==>
% see https://tex.stackexchange.com/questions/212362/how-to-use-declaresourcemap-to-add-default-value-to-a-field
\DeclareSourcemap{
	\maps[datatype=bibtex]{
		\map{% Will overwrite fields without the ``overwrite'' option
			\pertype{phdthesis}
			\step[fieldset=type, fieldvalue={Doctoral dissertation}]
		}
	}
}
% <==

% Remove superfluous ``The'' from journal names ==>
\DeclareSourcemap{ 
	\maps[datatype=bibtex]{
		\map{
			\step[fieldsource=journal, match={\regexp{^The\s}}, replace={}]
		}
	}      
}
% <==


==> templates/Preamble_BibLaTeX_APA.tex <==
% !TeX program = pdflatex
% !TeX TXS-program:compile = txs:///pdflatex/
% !TeX TS-program = pdflatex
% !BIB program = biber
% !TeX TXS-program:bibliography = txs:///biber




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  CITATION COMMANDS AND BIBLIOGRAPHY STYLE %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% For APA:
\usepackage[style=apa, backend=biber, natbib=true, backref=true]{biblatex}

\let\citeorig\cite
\renewcommand{\cite}{\citet}
\renewcommand{\citealp}{\citeorig}

\renewcommand{\bibfont}{\sffamily\small}
	% Reduce font size for the bibliography, make the font sans-serif.
\AtBeginDocument{%
	\setlength{\bibindent}{\parindent}%
}
\setlength{\bibitemsep}{0pt}

\DefineBibliographyStrings{english}{%
	backrefpage = {},	% originally ``cit. on p.''
	backrefpages = {}	% originally ``cit. on pp.''
}
\DefineBibliographyStrings{ngerman}{%
	backrefpage  = {},	% originally ``Siehe Seite''
	backrefpages = {}	% originally ``Siehe Seiten''
}

\renewcommand*{\finentrypunct}{}
\renewbibmacro*{pageref}{%
	\addperiod
	\iflistundef{pageref}
	{}
	{\printtext[brackets]{% NEW
			\ifnumgreater{\value{pageref}}{1}
			{\bibstring{backrefpages}}
			{\bibstring{backrefpage}}%
			\printlist[pageref][-\value{listtotal}]{pageref}%
		}%
	}%
}% NEW

% Link DOIs automatically to https://doi.org/<DOI>, in line with the
% APA's DOI Display Guidelines Update from March 2017:
% https://blog.apastyle.org/apastyle/digital-object-identifier-doi/
% ==>
\DeclareFieldFormat{doi}{%
	\Urlmuskip = 0mu\relax%
	\mathchardef\UrlBigBreakPenalty=1\relax%
	\mathchardef\UrlBreakPenalty=2\relax%
		% See https://tex.stackexchange.com/questions/22854/url-line-breaks-with-biblatex
	\url{https://doi.org/#1}%
}
% <==
\DeclareFieldFormat{url}{%
	\Urlmuskip = 0mu\relax%
	\mathchardef\UrlBigBreakPenalty=1\relax%
	\mathchardef\UrlBreakPenalty=2\relax%
		% See https://tex.stackexchange.com/questions/22854/url-line-breaks-with-biblatex
	\url{#1}%
}


==> templates/Preamble_Fonts_IBMPlex.tex <==
% !TeX TXS-program:compile = txs:///pdflatex/
% !TeX TS-program = pdflatex
% !TeX TXS-program:bibliography = txs:///biber
% !BIB program = biber




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  FONT SETTINGS AND TYPOGRAPHY  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Use Fira Sans as the sans-serif font.
% Load first because it otherwise doesn't work properly.
% ==>
%\usepackage[lining, scale=0.88]{FiraMono}  % To match the x-height of the Charter serif font
%\usepackage[book, semibold, lining, tabular, scale=0.88]{FiraSans}[2018/05/23]
%\makeatletter
%\@ifpackagelater{FiraSans}{2018/05/23}
%	{}
%	{\PackageError{FiraSans}
%	     {Outdated 'FiraSans' package}
%	     {Upgrade to FiraSans 2018/05/23 or newer!\MessageBreak
%	      Otherwise the sans-serif font may not work properly, or the compilation might fail.\MessageBreak
%	      This is a fatal error. I'm aborting now.}%
%	\endinput%
%   }
%\makeatother
%% In case you wish to use the ``light'' options of FiraSans: -->
%\ifthenelse{\isundefined{\AfterPackage}}{\usepackage{afterpackage}}{}
%\AfterPackage{siunitx}{%
%  \providecommand*{\lseries}{\fontseries{l}\selectfont}
%}
% See https://tex.stackexchange.com/questions/164791/combination-of-siunitx-and-light-weight-font-fails-to-compile.
% <--
% <==

\usepackage[xcharter, slantedGreek, scaled=1.055, upint]{newtxmath}
%\usepackage[xcharter, slantedGreek, scaled=1.09]{newtxmath}
% This template also works with the ``IBM Plex Sans'' and ``IBM Plex Mono'' fonts,
% https://ctan.org/pkg/plex ==>
\usepackage[textmd, semibold, scale=0.91]{plex-mono}  % To match the x-height of the Charter serif font
\usepackage[textmd, semibold, scale=0.91]{plex-sans}[2018/12/31]
% Earlier versions of the ``plex-sans'' package do not include support for LGR Greek.
% <==

%% This template also works with the ``Alegreya'' and ``Alegreya Sans'' fonts,
%% https://ctan.org/pkg/alegreya ==>
%\usepackage[semibold, scale=0.89]{plex-mono}  % To match the x-height of the Charter serif font
%\usepackage[lining, tabular, scale=1.02]{AlegreyaSans}[2018/08/02]
%	% Earlier versions of the ``Alegreya'' package do not include support for LGR Greek.
%% <==

%% This template also works with the ``Google Noto'' fonts,
%% https://ctan.org/pkg/noto ==>
%\usepackage[scale=0.85]{noto-mono}
%\usepackage[lining, tabular, scale=0.85]{noto-sans}[2019/01/11]
%	% Earlier versions of the ``noto'' package do not include support for LGR Greek.
%% <==

% Save the font family and font series definitions for later use: ==>
\newcommand{\savesffamily}{\sfdefault}
\makeatletter
\newcommand{\savesfmdseries}{\mdseries@sf}
\newcommand{\savesfbfseries}{\bfseries@sf}
\makeatother
% <==

% Use Bitstream Charter as the math font
% ==>
%\usepackage[charter, greeklowercase=italicized, greekuppercase=italicized, sfscaled=false, ttscaled=false]{mathdesign}
%% Use Alegreya as the text font -->
%\usepackage[lining, tabular, scale=1.02]{Alegreya}[2018/08/02]
%\ifxetex \else \DisableLigatures[T]{family = {rm*}} \fi
%% <--
%% Use Noto Serif as the text font -->
%\usepackage[lining, tabular, scale=0.85]{noto-serif}[2019/01/11]
%% <--
% Use IBM Plex as the text font -->
\usepackage[textmd, semibold, scale=0.91]{plex-serif}
% <--
% Save the font family and font series definitions for later use:
\let \savermfamily \rmdefault
\makeatletter
\newcommand{\savermmdseries}{\mdseries@rm}
\newcommand{\savermbfseries}{\bfseries@rm}
\makeatother
% <==

% mathdesign provides upright Greek letters as \alphaup, \Betaup, etc. while other packages
% (e.g., unicode-math) call these \upalpha, \upBeta, etc. We make also the latter available.
% ==>
\makeatletter
\@for\@tempa:=%
	alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,lambda,mu,nu,xi,%
	omicron,pi,rho,sigma,varsigma,tau,upsilon,phi,varphi,chi,psi,omega,digamma,%
	Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
	Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
\do{%
	\expandafter\let\csname up\@tempa\expandafter\endcsname\csname\@tempa up\endcsname%
}%
\makeatother
% <==

% Provide a \nequiv symbol
\ifx\nequiv\undefined
	\newcommand{\nequiv}{\not\equiv}
\fi

% Use Bitstream Charter as the text font
% ==>
%\usepackage[scaled=.96, lining, sups]{XCharter}  % option ``sups'' not working properly with subimport
% Save the font family and font series definitions for later use:
\let \savermdefaultfortext \rmdefault
\let \savemddefaultfortext \mddefault
\let \savebfdefaultfortext \bfdefault
\renewcommand{\textellipsis}{\mbox{.{\kern.09em}.{\kern.09em}.}}
%\makeatletter
%\newcommand{\@makefnmarkorig}{%
%	\hbox{\sufigures\hspace*{.04em}\@thefnmark\hspace*{.04em}}%
%}  % Copied from XCharter.sty
%\makeatother
% <==

\ifxetex
	% Do nothing.
\else
	\DisableLigatures[f]{family = {rm*, sf*, tt*}}
	% Disable the f* ligatures for the Plex fonts because the fonts do not provide sufficient support.
	% Disable the f* ligatures for the ``typewriter'' font because they make no sense for a monospaced font.
	\SetExtraKerning[unit=space]
		{encoding=*, family=*, series=*, size={*, normalsize, footnotesize}, font = */*/*/*/*}
		{\textemdash = {325, 325},
			/ = {100, 100},
			: = { 50,   0},
			; = { 50,   0}}
\fi

\usepackage{xfrac}	% Provides \sfrac

% Since math mode uses a different font encoding, issuing \euro/\texteuro in math mode
% produces an incorrect sign. We fix this. ==>
\AtBeginDocument{%
	\providecommand{\euro}[1]{%
		\relax\ifmmode\text{\texteuro}#1\else\texteuro #1\fi%
	}%
}
% <==


==> templates/Preamble_Fonts_Times.tex <==
% !TeX program = pdflatex
% !TeX TXS-program:compile = txs:///pdflatex/
% !TeX TS-program = pdflatex
% !BIB program = biber
% !TeX TXS-program:bibliography = txs:///biber




%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  FONT SETTINGS THESIS  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage{amsfonts, amssymb}  % Additional symbols from AMS

\usepackage{extarrows}

% Use Times Roman for text and math
\usepackage{newtxtext}
\usepackage[smallerops, varg, upint, slantedGreek]{newtxmath}

%\usepackage[scale=1.07]{tgcursor}
%	% Use Courier as the typewriter font
%\usepackage[scale=0.93]{sourcecodepro}
%	% Use Source Code Pro as the typewriter font
\usepackage[scaled=0.835]{DejaVuSansMono}  % Scaled to match the x-height of the newtxtext Times Roman
	% Use DejaVu Sans Mono as the typewriter font, also supports Greek via the LGR encoding

\usepackage{xfrac}

\usepackage[protrusion=true, expansion=false, kerning=true]{microtype}
% This package enables so-called hanging punctuation. That is, when a punctuation sign like ":", ".", "-", etc. is found at the beginning or end of a line, it is protruded a little into the page margin. This results in "optical margin alignment," because the protrusion makes the margin alignment look straighter.
%\DisableLigatures[f]{family = {sf*, rm*}}
%	% Disable the f* ligatures for both Fira Sans and Charter because both fonts provide insufficient support
%\DisableLigatures[f]{family = {rm*}}
	% Disable the f* ligatures for Charter because it provides insufficient support
\SetExtraKerning[unit=space]
{encoding=*, family=*, series=*, size={*, normalsize, footnotesize}, font = */*/*/*/*}
{\textemdash = {325, 325},
	/ = {100, 100},
	: = { 50,   0},
	; = { 50,   0}}
\renewcommand{\textellipsis}{\mbox{.{\kern.09em}.{\kern.09em}.}}

\renewcommand{\bibfont}{%
	\normalsize%
	\addtolength{\baselineskip}{0.05\baselineskip}%
	%\setlength{\baselineskip}{\newbaselineskip}%
}  % Use same size for bibliography as for body text.

\captionsetup{footfont={rm, footnotesize}}  % Set font in \floatfoot to serif and footnotesize




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  MATH-RELATED ADJUSTMENTS  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage{mathrsfs}  % Provides the \mathscr math alphabet

% The following is taken from
% https://tex.stackexchange.com/questions/116389/automatic-upright-math-when-text-is-in-italic/116399#116399
% Filling in ``missing'' Greek glyphs for completeness
% (not really necessary, since they look identical to Latin glyphs and are thus almost never used)
% ==>
\newcommand{\omicron}{o}
\newcommand{\Digamma}{F}
\newcommand{\Alpha}  {A}
\newcommand{\Beta}   {B}
\newcommand{\Epsilon}{E}
\newcommand{\Zeta}   {Z}
\newcommand{\Eta}    {H}
\newcommand{\Iota}   {I}
\newcommand{\Kappa}  {K}
\newcommand{\Mu}     {M}
\newcommand{\Nu}     {N}
\newcommand{\Omicron}{O}
\newcommand{\Rho}    {P}
\newcommand{\Tau}    {T}
\newcommand{\Chi}    {X}
% <==

% Upright Greek letters for the \mathup command
% ==>
\makeatletter
% Save original definitions of the Greek letters
\@for\@tempa:=%
	alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,lambda,mu,nu,xi,%
	omicron,pi,rho,sigma,varsigma,tau,upsilon,phi,chi,psi,omega,digamma,%
	Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
	Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
	\do{%
		\expandafter\let\csname\@tempa orig\expandafter\endcsname\csname\@tempa\endcsname%
		\expandafter\let\csname\@tempa uporig\expandafter\endcsname\csname\@tempa up\endcsname%
	}%
\newcommand*{\upgreekletters}{%
	\@for\@tempa:=%
		alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,lambda,mu,nu,xi,%
		omicron,pi,rho,sigma,varsigma,tau,upsilon,phi,chi,psi,omega,digamma,%
		Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
		Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
		\do{%
			\expandafter\let\csname\@tempa\expandafter\endcsname\csname\@tempa up\endcsname%
		}%
}
\newcommand*{\itgreekletters}{%
	\@for\@tempa:=%
		alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,lambda,mu,nu,xi,%
		omicron,pi,rho,sigma,varsigma,tau,upsilon,phi,chi,psi,omega,digamma,%
		Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
		Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
		\do{%
			\expandafter\let\csname\@tempa\expandafter\endcsname\csname\@tempa orig\endcsname%
		}%
}
\makeatother
% <==

\newcommand{\mathup}[1]{\upgreekletters\mathrm{#1}\itgreekletters}

\renewcommand{\mathbf}[1]{\bm{#1}}
\newcommand{\mathbfit}[1]{\mathbf{\mathit{#1}}}
\newcommand{\mathbfup}[1]{\upgreekletters\mathbf{\mathrm{#1}}\itgreekletters}

% Since math mode uses a different font encoding, issuing \euro/\texteuro in math mode
% produces an incorrect sign. We fix this. ==>
\AtBeginDocument{%
	\newcommand*{\euro}[1]{%
		\relax\ifmmode\text{\texteuro}#1\else\texteuro #1\fi%
	}%
}
% <==


==> templates/Preamble_Poster.tex <==
% !TeX program = pdflatex
% !TeX TXS-program:compile = txs:///pdflatex/
% !TeX TS-program = pdflatex
% !BIB program = biber
% !TeX TXS-program:bibliography = txs:///biber




%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  FUNDAMENTAL PACKAGES  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage[utf8]{inputenc}

\usepackage[LGR, T1]{fontenc}  % LGR needed for sansserif math

\usepackage[ngerman, american, USenglish]{babel}  % German and US English hyphenation and quotation marks
\selectlanguage{USenglish}

\usepackage{calc}  % Enables calculations for lengths
\usepackage[nomessages]{fp}	 % Enables calculations in LaTeX

\usepackage{etoolbox}  % Enables manipulating LaTeX commmands via \preto, \appto, \patchcmd, etc.
\usepackage{xpatch}  % Enables manipulating LaTeX commmands via \xpatchcmd etc.

\PassOptionsToPackage{cmyk}{xcolor}
\definecolor{UBonnBlue}  {cmyk}{1.00, 0.70, 0.00, 0.00}
\definecolor{UBonnYellow}{cmyk}{0.00, 0.20, 1.00, 0.00}
\definecolor{UBonnGray}  {cmyk}{0.00, 0.00, 0.15, 0.55}
\colorlet{SpotColor}{UBonnBlue}
\definecolor{CMYKBlack}{cmyk}{0.00, 0.00, 0.00, 1.00}
\colorlet{CMYKGray}{CMYKBlack!50!}
\setbeamercolor{normal text}{fg=CMYKBlack}
\setbeamercolor{alerted text}{fg=SpotColor}
\setbeamerfont{alerted text}{family=\sffamily, series=\bfseries}

\setbeamercolor{block alerted title}{bg=SpotColor, fg=white}
\setbeamercolor{block body}{fg=CMYKBlack}

\setbeamercolor{title in headline}{fg=SpotColor}
\setbeamercolor{institute in headline}{fg=CMYKBlack}

\hypersetup{
	colorlinks = false,
	urlcolor   = SpotColor,
	linkcolor  = SpotColor,
	citecolor  = SpotColor
}
\urlstyle{same}
\let \urlorig \url
\renewcommand{\url}[1]{\textcolor{SpotColor}{\urlorig{#1}}}
\let \hreforig \href
\renewcommand{\href}[2]{\textcolor{SpotColor}{\hreforig{#1}{#2}}}
\newcommand{\email}[1]{\href{mailto:#1}{\nolinkurl{#1}}}

\usepackage[absolute,overlay]{textpos}
\setlength{\TPboxrulesize}{1pt}
\textblockrulecolor{SpotColor}

\usepackage{ragged2e}

% microtype enables ``hanging punctuation'' and other neat microtypographic features
\ifxetex
	\usepackage[protrusion=true, expansion=false]{microtype}
\else
	\usepackage[protrusion=true, expansion=false, kerning=true]{microtype}
\fi

% Use the bm (= boldmath) package for better support of setting math in bold ==>
% Prevent the "Too many math fonts used" error:
\newcommand{\bmmax}{0}
\newcommand{\hmmax}{0}
\usepackage{bm}
% <==




%%%%%%%%%%%%%%%%%%%%%%%
%%  BEAMER SETTINGS  %%
%%%%%%%%%%%%%%%%%%%%%%%


% Use the beamerposter package for laying out the poster:
% \usepackage[size=a0, scale=1.1]{beamerposter}
	% A0: 840 mm by 1188 mm in beamerposter
\usepackage[size=custom, width=84.1, height=118.9, scale=1.2]{beamerposter}
	% 841 mm by 1189 mm: A0
\beamertemplatenavigationsymbolsempty

\usefonttheme{professionalfonts}

\newcommand{\highlight}[1]{\alert{\textbf{#1}}}

% Make itemize justified instead of flushleft
% ==>
\makeatletter
\renewcommand{\itemize}[1][]{%
	\beamer@ifempty{#1}{}{\def\beamer@defaultospec{#1}}%
	\ifnum \@itemdepth >2\relax\@toodeep\else
	\advance\@itemdepth\@ne
	\beamer@computepref\@itemdepth% sets \beameritemnestingprefix
	\usebeamerfont{itemize/enumerate \beameritemnestingprefix body}%
	\usebeamercolor[fg]{itemize/enumerate \beameritemnestingprefix body}%
	\usebeamertemplate{itemize/enumerate \beameritemnestingprefix body begin}%
	\list
	{\usebeamertemplate{itemize \beameritemnestingprefix item}}
	{\def\makelabel##1{%
			{%
				\hss\llap{{%
						\usebeamerfont*{itemize \beameritemnestingprefix item}%
						\usebeamercolor[fg]{itemize \beameritemnestingprefix item}##1}}%
			}%
		}%
	}
	\fi%
	\beamer@cramped%
	\justifying% NEW
	%\raggedright% ORIGINAL
	\beamer@firstlineitemizeunskip%
}
\makeatother
% <==

% Add white space before lists and between items inside lists
% ==>
\makeatletter
\def\@listi{\leftmargin\leftmarginii
	\topsep 0.333333\baselineskip % Spacing before lists
	\parsep 0\p@ \@plus\p@
	\itemsep 0.333333\baselineskip} % Spacing between items
\makeatother
% <==

\setbeamertemplate{itemize item}{\raisebox{-1.5pt}{\textbf{\textbullet}}}
\setbeamercolor{item}{fg=SpotColor}

\setbeamerfont{structure}{family=\sffamily, shape=\upshape, series=\bfseries}

\setbeamerfont{title}{series=\bfseries}
\setbeamercolor{title}{fg=SpotColor}

% Poster title
\setbeamertemplate{headline}{
	\leavevmode
	\begin{columns}
		\begin{column}{\linewidth}
			\vskip-0.6\topmargin
			% \centering
			\Huge\textbf{\textsf{\textcolor{SpotColor}{\inserttitle}}}\\[-57pt]
			{\color{SpotColor}\rule{\linewidth}{1pt}\\[-31pt]}
			\usebeamercolor{author in headline}{\Large\insertauthor}\\[-42pt]
			\usebeamercolor{institute in headline}{\large\textsf{\insertinstitute}}\\[1ex]
			\vskip1cm
		\end{column}
		\vspace{1cm}
	\end{columns}
	\vspace{0.5in}
	% \hspace{0.5in}\begin{beamercolorbox}[wd=47in,colsep=0.15cm]{cboxb}\end{beamercolorbox}
	% \hspace{\leftmargin}\rule{\textwidth-\leftmargin-\rightmargin}{0.4pt}
	\vspace{0.1in}
}

% Regular block definition
\setbeamerfont{block title}{family=\sffamily, series=\bfseries}
\setbeamercolor{block title}{fg=SpotColor}
\setbeamertemplate{block begin}{
	\par\vskip\medskipamount
	\begin{beamercolorbox}[colsep*=0ex, dp=30pt, left]{block title}
		\vskip-0.25cm
		\usebeamerfont{block title}%
		\large\insertblocktitle\\[-22pt]
		\rule{\linewidth}{1pt}\\[22pt]
	\end{beamercolorbox}
	{\parskip0pt\par}
	\ifbeamercolorempty[bg]{block title}
	{}
	{\ifbeamercolorempty[bg]{block body}{}{\nointerlineskip\vskip-0.5pt}}
	\usebeamerfont{block body}
	\vskip-0.75cm
	\begin{beamercolorbox}[colsep*=0ex,vmode]{block body}
		\setlength{\baselineskip}{36pt}%
		\sloppypar\justifying%
}
\setbeamertemplate{block end}{
	\end{beamercolorbox}
	\vskip\smallskipamount
}

% Alert block definition (with frame)
\setbeamerfont{block alerted title}{parent=structure, series=\fontseries{\savesfbfseries}\selectfont}
\newlength{\inboxwd}
\newlength{\iinboxwd}
\newlength{\inboxrule}
\setbeamertemplate{block alerted begin}{
  \par
  \begin{beamercolorbox}[sep=25pt, rounded=false, dp=2pt, leftskip=12pt, rightskip=12pt]{block alerted title}
    \usebeamerfont{block alerted title}%
    {\sloppy\large\insertblocktitle}
  \end{beamercolorbox}
  {\parskip0pt\par}
  \usebeamerfont{block body}
  \vskip-0.25in
  \begin{beamercolorbox}[sep=0.5cm, rounded=false, center]{block body}
  \setlength{\inboxwd}{\linewidth}
  \addtolength{\inboxwd}{-1cm}
  \begin{beamercolorbox}[rounded=false, wd={\inboxwd}, center]{block body}
  \setlength{\iinboxwd}{\inboxwd}
  \setlength{\inboxrule}{\inboxwd}
  \addtolength{\iinboxwd}{-0.5cm}
  \addtolength{\inboxrule}{0.5cm}
  \begin{center}
  \begin{minipage}{\iinboxwd}
  \centering%
  \sffamily
}
\setbeamertemplate{block alerted end}{
  \end{minipage}
  \end{center}
  \end{beamercolorbox}
  \end{beamercolorbox}
  \vskip\smallskipamount
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  BIBLIOGRAPHY SETTINGS  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\usepackage{natbib}
\newlength{\bibindent}
\newlength{\bibitemsep}
\newlength{\bibsep}

\setbeamertemplate{bibliography item}{}
\setbeamercolor{bibliography entry author}  {fg=SpotColor}
\setbeamercolor{bibliography entry title}   {fg=SpotColor}
\setbeamercolor{bibliography entry location}{fg=SpotColor}
\setbeamercolor{bibliography entry note}    {fg=SpotColor}




%%%%%%%%%%%%%%%%%%%%%
%%  MISCELLANEOUS  %%
%%%%%%%%%%%%%%%%%%%%%


\newcommand{\affilindicator}[1]{\textsuperscript{\kern.75pt \textit{#1}}}
\usepackage[math]{blindtext}  % For debugging only
\makeatletter
\def\blindtext@american{}
\makeatother

% Allow for fine-grained scaling of font sizes
% ==>
\usepackage{relsize}
\renewcommand\RSpercentTolerance{1}
% Enabling slightly reduced font for CAPS:
\newcommand{\caps}[1]{\textscale{0.96}{\textls[35]{\MakeUppercase{#1}}}}
% <==




%%%%%%%%%%%%%%%%%%%%%%%
%%  DOCUMENT LAYOUT  %%
%%%%%%%%%%%%%%%%%%%%%%%


\setlength{\leftmargin}{4cm}
\setlength{\rightmargin}{4cm}

\newenvironment{parblock}[1]%
	{\begin{block}{#1}%
	 \setlength{\parindent}{\baselinestretch\baselineskip}%
	 \noindent\ignorespaces%
	}%
	{\end{block}}

\newcommand{\numcols}{3}
\FPeval{\numcolsminusone}{\numcols-1}

\newlength{\colsep}
\setlength{\colsep}{1.5cm}
\newlength{\totalcolsep}
\setlength{\totalcolsep}{\numcolsminusone\colsep}

\newlength{\colwidth}
\setlength{\colwidth}{(\paperwidth-\leftmargin-\rightmargin-\totalcolsep)/\numcols}

\setbeamersize{text margin left=\leftmargin, text margin right=\rightmargin}

\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{1pt}%

\frenchspacing


==> templates/Preamble_Presentation.tex <==
% !TeX program = pdflatex
% !TeX TXS-program:compile = txs:///pdflatex/
% !TeX TS-program = pdflatex
% !BIB program = biber
% !TeX TXS-program:bibliography = txs:///biber




%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  FUNDAMENTAL SETTINGS  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\serifbodyfont}{0}
% 0: Body is set in sans-serif font
% 1: Body is set in serif font
\newcommand{\serifheadingfont}{0}
% 0: Headings (``structure'') are set in sans-serif font
% 1: Headings (``structure'') are set in serif font

\newcommand{\showsectionnavigation}{0}
% 0: ``Headline'' is disabled.
% 1: ``Headline'' (at the very top of slides) is included and displays all sections of the presentation,
%      with the current section being highlighted.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  FUNDAMENTAL PACKAGES  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage{ifthen}

\usepackage{calc}

\usepackage{tcolorbox}

\usepackage[LY1, LGR, TS1, T1]{fontenc}
% LGR (Greek) is needed to enable the ``sansserif math'' features.
\usepackage[utf8]{inputenc}

\usepackage{tabularx}

\ifxetex
	\usepackage[protrusion=true, expansion=false]{microtype}
\else
	\usepackage[protrusion=true, expansion=false, kerning=true]{microtype}
\fi
% The microtype package enables so-called hanging punctuation. That is, when a punctuation sign like ":", ".", "-", etc. is found at the beginning or end of a line, it is protruded a little into the page margin. This results in "optical margin alignment," because the protrusion makes the margin alignment look straighter.


\definecolor{darkgray}{rgb}{0.4,0.4,0.4}

\usepackage[absolute, overlay]{textpos}
\usepackage{graphicx}
\usepackage{amsmath}
%\usepackage{amsfonts}
%\usepackage{amssymb}
\usepackage{epstopdf}
\DeclareGraphicsRule{.tif}{png}{.png}{`convert #1 `dirname #1`/`basename #1 .tif`.png}

\usepackage[ngerman, american, USenglish]{babel}
% German and US English hyphenation and quotation marks
\selectlanguage{USenglish}
\usepackage[autostyle=true]{csquotes}

\usepackage{multirow}

\usepackage{xcolor}
\usepackage{pgf}%,pgfarrows,pgfnodes,pgfshade}
\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{mindmap, trees, patterns}

\usepackage{xspace}

% \usepackage{eurosym}

%\usepackage{etoolbox}
%	% Enables manipulating LaTeX commmands via \preto, \appto, \patchcmd, etc.
%	% loaded automatically by beamer
\usepackage{xpatch}
% Enables manipulating LaTeX commmands via \xpatchcmd etc.

\hypersetup{%
	pdfpagemode=FullScreen,
	breaklinks=true,
	colorlinks, linkcolor=, urlcolor=SpotColor, citecolor=%
}
\urlstyle{same}
\newcommand{\email}[1]{\href{mailto:#1}{\nolinkurl{#1}}}

\usepackage{import}	 % To allow for relative paths in nested \input's (\import's)




%%%%%%%%%%%%%%%%%%%%%
%%  FONT SETTINGS  %%
%%%%%%%%%%%%%%%%%%%%%


\subimport{0_0_Preamble/}{Preamble_Fonts_Charter_FiraSans}

\ifnum \serifbodyfont=0
	\setbeamerfont{normal text}{family=\sffamily}
	\renewcommand{\familydefault}{\savesffamily}
	\renewcommand{\mddefault}{\savesfmdseries}
	\renewcommand{\bfdefault}{\savesfbfseries}
\else
	\usefonttheme{serif}
	\setbeamerfont{normal text}{family=\rmfamily}
\fi
\ifnum \serifheadingfont=0
	\setbeamerfont{structure}{family=\sffamily, shape=\upshape, series=\bfseries}
\else
	\setbeamerfont{structure}{family=\rmfamily, shape=\upshape, series=\bfseries}
\fi

% Make frame titles and headings bold
\usefonttheme{structurebold}
\usefonttheme{professionalfonts}

\setbeamerfont{footline}
	{parent=structure, size=\tiny, series=\mdseries}
\setbeamercolor{footline}
	{fg=SpotColor}

%% Use the bm (= boldmath) package for better support of setting math in bold ==>
%% Prevent the "Too many math fonts used" error:
\newcommand{\bmmax}{0}
\newcommand{\hmmax}{0}
\usepackage{bm}
%% <==

\usepackage{fontawesome}

\usepackage{mathtools}
%\mathtoolsset{centercolon}
% This makes the compilation fail in combination with tikz. See
% https://tex.stackexchange.com/questions/89467/why-does-pdftex-hang-on-this-file.
%% Inspired by https://tex.stackexchange.com/questions/251460/how-to-put-symbols-of-equal-size-on-top-of-each-other
\newcommand{\succeqq}{%
	\mathrel{%
		\vcenter{\offinterlineskip
			\ialign{##\cr$\succ$\cr\noalign{\kern 1pt}$=$\cr}%
		}%
	}%
}
\newcommand{\nsucceqq}{\mathrel{\not\succeqq}}
\newcommand*{\coloneqq}{\mathrel{%
		\mathrel{%
			\raisebox{0.15ex}{\scalebox{0.85}{\ensuremath{:}}}\hspace{-0.2pt}%
		}%
		=%
}}

\input{0_0_Preamble/Preamble_Sansserif_math}

% Allow for fine-grained scaling of font sizes
% ==>
\usepackage{relsize}
\renewcommand\RSpercentTolerance{1}
% Enabling slightly reduced font for CAPS:
\newcommand{\caps}[1]{\textscale{0.96}{\textls[35]{\MakeUppercase{#1}}}}
% <==




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  ADJUSTING THE DESIGN OF THE PRESENTATION  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\setbeamerfont{title}
	{parent=structure, size=\LARGE, series=\bfseries}
\setbeamerfont{subtitle}
	{parent=structure, size=\Large, series=\mdseries}
\setbeamerfont{frametitle}
	{parent=structure, size=\large}

% For convenience, let the ``paperheight'' of the slides be identical,
% no matter what the aspect ratio of the slides ==>
\makeatletter
% 4:3 aspect ratio:
\@ifclasswith{beamer}{aspectratio=43}{%
	\beamer@paperwidth 12.00cm%
	\beamer@paperheight 9.00cm%
	\setbeamerfont{title}
		{parent=structure, size*={16}{20}}
	\setbeamerfont{subtitle}
		{parent=structure, size*={13.5}{17}}
	\setbeamerfont{frametitle}
		{parent=structure, size*={11}{14}}
}{}
%% 14:9 aspect ratio: Nothing needs to be changed
%\@ifclasswith{beamer}{aspectratio=149}{%
%	\beamer@paperwidth 14.00cm%
%	\beamer@paperheight 9.00cm%
%}{}
%% 16:9 aspect ratio: Nothing needs to be changed
%\@ifclasswith{beamer}{aspectratio=169}{%
%	\beamer@paperwidth 16.00cm%
%	\beamer@paperheight 9.00cm%
%}{}
% 16:10 aspect ratio:
\@ifclasswith{beamer}{aspectratio=1610}{%
	\beamer@paperwidth 14.40cm%
	\beamer@paperheight 9.00cm%
}{}
\makeatother
% <==

% Margins ==>
\newcommand{\margintop}{12.5pt}
\newcommand{\marginleft}{17.5pt}
\newcommand{\marginright}{\marginleft}
\setbeamersize{text margin left=\marginleft}
\setbeamersize{text margin right=\marginright}
\setlength{\textwidth}{\paperwidth-\marginleft-\marginright}
% <==

\setlength{\parskip}{\medskipamount}
% Inserts some space between paragraphs

% Enable hyphenation on Beamer slides:
\usepackage{ragged2e}
\let \raggedright \RaggedRight
\sloppy
\hyphenpenalty=500

\setbeamerfont{alerted text}{series=\bfseries}

%% Lorenz Götte's color scheme:
%\usecolortheme{whale}
%\definecolor{beamer@blendedblue}{rgb}{0.137,0.466,0.741}
%\setbeamercolor{structure}{fg=beamer@blendedblue}
%\definecolor{SpotColor}{rgb}{0.1,0.4,0.7} % Lorenz' Blue
\definecolor{UBonnBlue}   {RGB}{  7,  82, 154}
\definecolor{UBonnYellow} {RGB}{234, 185,  12}
\definecolor{UBonnGray}   {RGB}{144, 144, 133}
\definecolor{darkgray}    {RGB}{102, 102, 102}
\definecolor{darkred}     {RGB}{191,   0,   0}
\definecolor{neutralgreen}{RGB}{ 28, 166,   0}

\colorlet{SpotColor}   {UBonnBlue}
\colorlet{AlertColor}  {darkred}
\colorlet{ExampleColor}{neutralgreen}

\setbeamercolor{structure}{fg=SpotColor}
\setbeamercolor{alerted text}{fg=AlertColor}
\setbeamercolor{author in head/foot}{fg=white, bg=SpotColor}
\setbeamercolor{button}{bg=SpotColor,fg=white}
\setbeamercolor{headline}{bg=SpotColor,fg=white}
\setbeamercolor{headlinecover}{bg=white,fg=white}

\newcommand{\highlight}[1]{\textcolor{SpotColor}{#1}}
\newcommand{\heading}[1]{%
	\par%
	\textbf{\usebeamerfont{structure}\usebeamercolor[fg]{frametitle}#1}%
	\par%
}
\newcommand{\sigstar}{\highlight{*}}

\renewcommand{\alert}[1]{\highlight{\textbf{#1}}}

\newlength{\rulelength}
\setlength{\rulelength}{\paperwidth - \marginleft - \marginright}
\newcommand{\sliderule}{%
	\textcolor{SpotColor}{\rule{\rulelength}{.35pt}}%
}

% Remove navigation symbols from the slide footer
\beamertemplatenavigationsymbolsempty

% Adjust layout of frametitle
% ==>
\setbeamertemplate{frametitle}{%
	\vspace{\margintop}\vspace{-5pt}%
	{\large\usebeamercolor{frametitle}\usebeamerfont{frametitle}\insertframetitle\\[-1.2ex]}%
	\sliderule\vspace{-2.5pt}%
}
% <==

\newlength{\navigationwidth}
\BeforeBeginEnvironment{frame}{%
	% Add a slide number (and [short]title) to the footer of each slide
	% ==>
	\setbeamertemplate{footline}{\vskip-15pt%
		\hspace{\marginleft}%
		\sliderule \vspace{1.1ex} \linebreak
		\mbox{\hspace{\marginleft}}%
		\textmd{\insertshortauthor: \enquote{\insertshorttitle}}
		\hfill%
		\textbf{\insertframenumber/\inserttotalframenumber}%
		\hspace{\marginright}%
		\vspace{12pt}%
	}%
	% <==
	% Outline with current section highlighted in the ``headline'' ==>
	\ifnum \showsectionnavigation=0
	\setbeamertemplate{headline}{}
	\else
	\setbeamertemplate{headline}{%
		\hspace{\marginleft}%
		\begin{beamercolorbox}[wd=\linewidth, ht=5pt, dp=2pt]{headline}%
			\insertsectionnavigationhorizontal{\linewidth}{\hspace{0.04\linewidth}}{\hspace{0.04\linewidth}}%
		\end{beamercolorbox}%
		\newline
		\begin{beamercolorbox}[wd=\paperwidth, ht=15pt, dp=0pt]{headlinecover}%
			% Adds a white bar to cover stuff that protrudes from the above color box.
		\end{beamercolorbox}%
	}
	\setlength{\fboxrule}{0.25pt}\setlength{\fboxsep}{7.5pt}%
	\setbeamertemplate{section in head/foot}{%
		\settowidth{\navigationwidth}{\bfseries\insertsectionhead}%
		\fcolorbox{SpotColor!25}{SpotColor}{%
			\makebox[\navigationwidth]{\color{white}\bfseries\insertsectionhead}%
		}%
	}
	\setbeamertemplate{section in head/foot shaded}{%
		\settowidth{\navigationwidth}{\bfseries\insertsectionhead}%
		\fcolorbox{SpotColor}{SpotColor}{%
			\makebox[\navigationwidth]{\color{white}\mdseries\insertsectionhead}%
		}
	}
	\fi
	% <==
}

% See https://tex.stackexchange.com/questions/427257/how-to-remove-footer-for-specific-type-of-slides-frames
% ==>
\makeatletter
\define@key{beamerframe}{standout}[true]{%
	\setbeamertemplate{footline}{\vskip-15pt%
		\hspace{\marginleft}%
		\sliderule \vspace{1.1ex} \linebreak
		\mbox{\hspace{\marginleft}}%
		\textmd{\phantom{\insertshortauthor: \enquote{\insertshorttitle}}}
		\hfill%
		\phantom{\insertframenumber/\inserttotalframenumber}%
		\hspace{\marginright}%
		\vspace{15pt}%
	}%
	\setbeamertemplate{headline}{}%
}
\makeatother
% <==

\frenchspacing  % Prevent increased whitespace after periods and colons

\setbeamertemplate{button}{%
	\tikz
	\node[
	inner xsep=3pt,
	inner ysep=2pt,
	draw=structure!100,
	fill=structure!100,
	rounded corners=1.5pt
	]{\raisebox{1.5pt}{\usebeamerfont{structure}\insertbuttontext}};%
}

%\renewcommand{\texteuro}{\fontencoding{TS1}\selectfont\char"BF\fontencoding{T1}\selectfont}
%\newcommand{\euro}{\texteuro}

% Adding framenumbers automatically to the frametitles
\newcommand{\pageinsection}{\number\numexpr\insertpagenumber-\insertsectionstartpage+1}
% From https://tex.stackexchange.com/questions/308343/how-to-create-mini-sections-mini-subsections-and-mini-frames-in-beamer-presenta
% ==>
%\usepackage{etoolbox}  % Automatically loaded by beamer
\makeatletter
\newcount\beamer@sectionstartframe
\beamer@sectionstartframe=1
\apptocmd{\beamer@section}{%
	\addtocontents{nav}{\protect\headcommand{%
			\protect\beamer@sectionframes{\the\beamer@sectionstartframe}{\the\c@framenumber}}}%
}{}{}
\apptocmd{\beamer@section}{%
	\beamer@sectionstartframe=\c@framenumber\advance\beamer@sectionstartframe by1\relax%
}{}{}
\AtEndDocument{%
	\immediate\write\@auxout{\string\@writefile{nav}%
		{\noexpand\headcommand{\noexpand\beamer@sectionframes{\the\beamer@sectionstartframe}{\the\c@framenumber}}}}%
}{}{}
\def\beamer@startframeofsection{1}
\def\beamer@endframeofsection{1}
\def\beamer@sectionframes#1#2{%
	\ifnum\c@framenumber<#1%
	\else%
	\ifnum\c@framenumber>#2%
	\else%
	\gdef\beamer@startframeofsection{#1}%
	\gdef\beamer@endframeofsection{#2}%
	\fi%
	\fi%
}
\newcommand\insertsectionstartframe{\beamer@startframeofsection}
\newcommand\insertsectionendframe{\beamer@endframeofsection}
\makeatother
% <==
\newcommand{\frameinsection}{\number\numexpr\insertframenumber-\insertsectionstartframe+1}
% https://tex.stackexchange.com/questions/228684/two-counters-for-beamer-presentations
%\newcommand{\titleprefix}{\insertsection~{\pageinsection}}
\newcommand{\titleprefix}{\insertsection~{\frameinsection}}
% <==

% Continuation counter for frames with the ``allowframebreaks'' option.
% ==>
%% Inspired by https://tex.stackexchange.com/questions/275044/how-do-i-insert-the-total-continuation-count-in-the-allowframbreaks-frame-title:
%\newcounter{totalcontinuationcount}
%\makeatletter
%\setbeamertemplate{frametitle continuation}{%
%	\setcounter{totalcontinuationcount}{\beamer@endpageofframe}%
%	\addtocounter{totalcontinuationcount}{1}%
%	\addtocounter{totalcontinuationcount}{-\beamer@startpageofframe}%
%	\ifnum \value{totalcontinuationcount} > 1
%		\textmd{(\insertcontinuationcount/\arabic{totalcontinuationcount})}%
%	\fi
%}
%\makeatother
% More elegant version based on https://github.com/josephwright/beamer/issues/423#issuecomment-456494500:
\makeatletter
\defbeamertemplate*{frametitle continuation}{only if multiple}{%
	\ifnum \numexpr\beamer@endpageofframe+1-\beamer@startpageofframe\relax > 1
	\textmd{(%
		\insertcontinuationcount/%
		\the\numexpr\beamer@endpageofframe+1-\beamer@startpageofframe%
		)}%
	\fi%
}
\makeatother
% <==




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  LAYOUT OF THE TITLE SLIDE  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Make the title page left-aligned
% ==>
%\setbeamertemplate{title page}[default][left]

% \setbeamerfont{title} and \setbeamerfont{subtitle} already executed above!
\setbeamerfont{author}
	{parent=normal text, size=\large, series=\mdseries, shape=\upshape}
\setbeamercolor{author}
	{parent=normal text}
\setbeamerfont{institute}
	{parent=normal text, size=\small, series=\mdseries, shape=\itshape}
\setbeamercolor{institute}
	{parent=normal text}
\setbeamerfont{date}
	{parent=structure, size=\normalsize, series=\bfseries}
\setbeamercolor{date}
	{parent=normal text}

\makeatletter
\setbeamertemplate{title page}{
	\begin{minipage}[c][6.75cm]{\textwidth}%
		\raggedright%
		\ifx\inserttitlegraphic\@empty\else%
			\inserttitlegraphic%
		\fi
		\vfill
		\begingroup
			\ifx\inserttitle\@empty\else%
				\usebeamerfont{title}\usebeamercolor[fg]{title}\inserttitle\par%
			\fi
			\ifx\insertsubtitle\@empty\else%
				\medskip
				\usebeamerfont{subtitle}\usebeamercolor[fg]{subtitle}\insertsubtitle\par%
			\fi
			\ifx\beamer@shortauthor\@empty\else%
				\vspace{\fill}
				\usebeamerfont{author}\usebeamercolor[fg]{author}\insertauthor\par%
			\fi
			\ifx\insertinstitute\@empty\else%
				\vspace{\fill}
				\usebeamerfont{institute}\usebeamercolor[fg]{institute}\insertinstitute\par%
			\fi
			\ifx\insertdate\@empty\else%
				\vspace{\fill}
				\usebeamerfont{date}\usebeamercolor[fg]{date}\insertdate%
			\fi
		\endgroup
		\vfill
		\vspace{0cm}  % For the \vfill to actually have an effect
	\end{minipage}%
}
\makeatother
% <==

\makeatletter
\renewcommand{\beamer@insttitle}[1]{\highlight{\textsuperscript{\kern.75pt \textit{#1}}}}
\renewcommand{\beamer@instinst}[1]{\beamer@insttitle{#1}\ignorespaces}
\renewcommand{\beamer@andinst}{\\[0.33\baselineskip]}
\makeatother




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  LAYOUT OF THE TABLE OF CONTENTS  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\useinnertheme{circles}
\setbeamertemplate{section in toc}{%
	\leavevmode\leftskip=3.3ex%
	\llap{%
		\usebeamerfont*{section number projected}%
		\usebeamercolor{section number projected}%
		\begin{pgfpicture}{-1ex}{0ex}{1ex}{2ex}
			\color{bg}
			\pgfpathcircle{\pgfpoint{0pt}{.75ex}}{1.2ex}
			\pgfusepath{fill}
			\pgftext[base]{\color{fg}\raisebox{0.07ex}{%
					% \addfontfeatures{Numbers={Lining, Monospaced}}%
					\usebeamerfont{structure}%
					\small\inserttocsectionnumber}%
			}
		\end{pgfpicture}\kern1.5ex%
	}%
	\usebeamerfont{normal text}%
	\inserttocsection\par%
}
\setbeamertemplate{subsection in toc}{%
	\leavevmode\leftskip=2em$\bullet$\hskip1em\inserttocsubsection\par%
}

\makeatletter
\patchcmd{\beamer@sectionintoc}
{\vfill}
{\medskip}
{}
{}
\makeatother




%%%%%%%%%%%%%%
%%  BLOCKS  %%
%%%%%%%%%%%%%%


% Put border around block, exampleblock, and alertblock
% ==>

\usepackage{mdframed}
\usepackage{changepage}

\newlength{\blockinnermargin}
\setlength{\blockinnermargin}{4pt}

\newcommand{\framedblockcolor}{SpotColor}  % This allows us to change the color mid-presentation
\newcommand{\PutBorderAroundBlock}[2]{
	\renewcommand{\framedblockcolor}{#2}%
	\setbeamercolor*{block title}{fg=white, bg=\framedblockcolor}%
	\setbeamercolor*{block body} {fg=black, bg=}%
	\addtobeamertemplate{block begin}{%
		\setbeamercolor*{item}{fg=\framedblockcolor}%
		\begin{mdframed}[linecolor=\framedblockcolor, linewidth=0.35pt, leftmargin=0pt, innerleftmargin=0.375em, innerrightmargin=0.375em, innertopmargin=-0.01ex, innerbottommargin=4pt]%
			\let \insertblocktitleorig \insertblocktitle%
			\renewcommand{\insertblocktitle}{%
				\RaggedRight%
				\leftskip=\blockinnermargin%
				\rightskip=\blockinnermargin%
				\insertblocktitleorig\strut\vspace{-1.5pt}%
					% \strut\vspace{-1.5pt} so that all single-line block titles have identical hight
			}%
	}{%
		\renewcommand{\insertblocktitle}{\insertblocktitleorig}%
		\begin{adjustwidth}{\blockinnermargin}{\blockinnermargin}%
			\RaggedRight%
	}%
	\addtobeamertemplate{block end}{%
		\end{adjustwidth}%
	}{%
		\end{mdframed}%
	}%
}
\PutBorderAroundBlock{}{SpotColor}  % Default color of blocks is SpotColor

\newcommand{\PutBorderAroundBlockExAlert}[2]{%
	\def\temp{#1}%
	\ifx\temp\empty
		\def\blocktype{block }     % Trailing space is crucial!
	\else
		\def\temp{ #1}
		\def\blocktype{block #1 }  % Trailing space is crucial!
	\fi
	\setbeamercolor*{block title\temp}{fg=white, bg=#2}
	\setbeamercolor*{block body\temp} {fg=black, bg=}
	\addtobeamertemplate{\blocktype begin}{%
		\begin{mdframed}[linecolor=#2, linewidth=0.35pt, leftmargin=0pt, innerleftmargin=0.375em, innerrightmargin=0.375em, innertopmargin=-0.01ex, innerbottommargin=4pt]%
			\let \insertblocktitleorig \insertblocktitle%
			\renewcommand{\insertblocktitle}{%
				\RaggedRight%
				\leftskip=\blockinnermargin%
				\rightskip=\blockinnermargin%
				\insertblocktitleorig\strut\vspace{-1.5pt}%
					% \strut\vspace{-1.5pt} so that all single-line block titles have identical hight
			}%
	}{%
		\renewcommand{\insertblocktitle}{\insertblocktitleorig}%
		\begin{adjustwidth}{\blockinnermargin}{\blockinnermargin}%
			\RaggedRight%
	}%
	\addtobeamertemplate{\blocktype end}{%
		\end{adjustwidth}%
	}{%
		\end{mdframed}%
	}%
}
\PutBorderAroundBlockExAlert{example}{ExampleColor}
\PutBorderAroundBlockExAlert{alerted}{AlertColor}

% <==

% Style definition, theorem, lemma, corollary, and proof with out border
% ==>

% Inspired by https://github.com/schnorr/infufrgs/blob/master/slides/beamerthemeInf.sty
\setbeamercolor{theorem title}{fg=SpotColor}
\setbeamerfont{theorem title}{parent=structure}
\setbeamercolor{theorem body}{fg=black}
\setbeamerfont{theorem body}{parent=normal text, shape=\itshape, series=\mdseries}
% Body of theorem, lemma, and corollary are italicized
\AtBeginEnvironment{definition}{%
	\setbeamerfont{theorem body}{parent=normal text, shape=\upshape, series=\mdseries}
	% Body of definition is typeset in upright font
}

\setbeamertemplate{theorem begin}{%
	\usebeamerfont{theorem title}%
	\usebeamercolor[fg]{theorem title}%
	\inserttheoremname%~\inserttheoremnumber%
	\ifx\inserttheoremaddition\empty\else\ (\inserttheoremaddition)\fi%
	%\inserttheorempunctuation\hspace{1ex}%
	\\[\smallskipamount]
	\usebeamerfont{theorem body}%
	\usebeamercolor[fg]{theorem body}%
}
\setbeamertemplate{theorem end}{}

\setbeamercolor{proof title}{fg=SpotColor}
\setbeamerfont {proof title}{parent=structure}
\setbeamercolor{proof body} {fg=black}
\setbeamerfont {proof body} {parent=normal text, shape=\upshape, series=\mdseries}
% Remove period after ``Proof''
% See https://tex.stackexchange.com/questions/31354/how-to-remove-the-in-the-proof-environment
% -->
\makeatletter
\let\@addpunct\@gobble
\makeatother
% <--
\renewcommand{\qedsymbol}{\small\textcolor{SpotColor}{$\blacksquare$}}
\setbeamertemplate{proof begin}{%
	\usebeamerfont{proof title}%
	\usebeamercolor[fg]{theorem title}%
	\insertproofname\\[\smallskipamount]
	\usebeamerfont{proof body}%
	\usebeamercolor[fg]{proof body}%
}
\setbeamertemplate{proof end}{}

% <==




%%%%%%%%%%%%%
%%  LISTS  %%
%%%%%%%%%%%%%


\AtBeginEnvironment{itemize}{%
	\setlength{\partopsep}{-\smallskipamount}%
	\setlength{\labelsep}{0.55em}%
	\setlength{\labelwidth}{\widthof{9.}}%
}
\AtBeginEnvironment{enumerate}{%
	\setlength{\partopsep}{-\smallskipamount}%
	\setlength{\labelsep}{0.5em}%
	\setlength{\labelwidth}{\widthof{9.}}%
}

% Adjust spacing of lists ==>
% Unfortunately, the ``enumitem'' package is incompatible with the ``beamer'' class.
% Hence, we need to adjust left margins etc. manually:
\setlength{\leftmargini}{\widthof{9.}+\labelsep}
\setlength{\leftmarginii}{\widthof{g.}+\labelsep}
\setlength{\leftmarginiii}{\widthof{iii.}+\labelsep}
%\setlength{\rightmargin}{0in}
%\setlength{\itemindent}{0in}
%\usepackage{enumitem}
%\setlist[enumerate, 1]{
%	leftmargin=-\parindent, listparindent=\parindent, labelsep=0.42\parindent, itemsep=\smallskipamount, parsep=0pt
%}
%
%\setlist[itemize, 1]{
%	leftmargin=0pt, listparindent=\parindent, labelsep=0.75em, itemsep=\smallskipamount, parsep=0pt, topsep=1.2ex, label=\usebeamerfont*{itemize item}	\usebeamercolor[fg]{itemize item} \usebeamertemplate{itemize item}, before={\RaggedRight \hyphenpenalty=1000}
%}
%\setlist[itemize, 2]{
%	leftmargin=1.2em, listparindent=\parindent, labelsep=0.6em, itemsep=\smallskipamount, parsep=0pt, topsep=0.6ex, label=\usebeamercolor[fg]{itemize item} --, before={\RaggedRight \hyphenpenalty=1000}
%}
% <==

% ``Medium'' as the bold series:
%\makeatletter
%\def\bfseries@sf{mb}
%\makeatother

%\useinnertheme{circles}

\setbeamertemplate{enumerate items}
[default]
\setbeamertemplate{enumerate subitem}
{\alph{enumii}.}
\setbeamertemplate{enumerate subsubitem}
{\roman{enumiii}.}

\setbeamertemplate{itemize item}
{\raisebox{-0.5pt}{\scalebox{0.95}{\textrm{\textbf{\textbullet}}}}\hspace{-0.06em}}
\setbeamertemplate{itemize subitem}
{\usebeamerfont{normal text}--\hspace{0.15em}}
\setbeamertemplate{itemize subsubitem}
{\raisebox{1.5pt}{\tiny$\blacktriangleright$}\hspace{0.15em}}

\setbeamerfont*{itemize/enumerate body}{size=\normalsize}
\setbeamerfont*{itemize/enumerate subbody}{parent=itemize/enumerate body}
\setbeamerfont*{itemize/enumerate subsubbody}{parent=itemize/enumerate body}

\renewenvironment{quote}{%
	\list{}{\leftmargin\leftmarginii \rightmargin\leftmarginii}%
	\RaggedLeft
	\itshape%
	\item\relax%
}
{\endlist}




%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  FIGURES AND TABLES  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%


\setbeamertemplate{caption}[numbered]
\setbeamertemplate{caption label separator}{. }
\usepackage[justification=centering]{caption}
\ifnum \serifbodyfont=0
	\captionsetup{font={sf, small}}
\else
	\captionsetup{font={rm, small}}
\fi
\ifnum \serifheadingfont=0
	\captionsetup{labelfont={sf, small, bf, color=SpotColor}}
\else
	\captionsetup{labelfont={rm, small, bf, color=SpotColor}}
\fi

\usepackage{tabularx}	% Provides environment tabularx to adjust width of tables
% \usepackage{tabulary}	% For some reason, tabulary doesn't obey the width argument ...
% Emulate the "tabulary" column types:
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{J}{>{\arraybackslash}X}
\newcolumntype{L}{>{\RaggedRight\arraybackslash}X}
\newcolumntype{R}{>{\RaggedLeft\arraybackslash}X}
% \usepackage[flushleft]{threeparttable}	% Provides the tablenotes environment


% Packages for creating better-looking tables
\usepackage{booktabs}
\setlength{\cmidrulewidth}{.35pt}
\setlength{\lightrulewidth}{.35pt}
\setlength{\heavyrulewidth}{.70pt}
\setlength{\abovetopsep}{-8pt}
\addtolength{\aboverulesep}{1pt}	% Make tables a little more spacious
\addtolength{\belowrulesep}{1pt}
% \setlength{\belowbottomsep}{-2pt}
\usepackage{colortbl} % e.g., for colored rules
\arrayrulecolor{SpotColor} % Color all table rules blue

\usepackage{siunitx}
% Allows, among others, for alignment of decimal numbers in tables at the decimal point.
\sisetup{
	detect-all,
	round-integer-to-decimal = true,
	group-digits             = true,
	group-minimum-digits     = 5,
	group-separator          = {\kern 1pt},
	table-align-text-pre     = false,
	table-align-text-post    = false,
	input-signs              = + -,
	input-symbols            = {*} {**} {***} \sigstar,
	input-open-uncertainty 	 = ,
	input-close-uncertainty  = ,
	retain-explicit-plus
}
\newcolumntype{T}[1]
{@{}S[table-format = #1, table-space-text-pre = {***}, table-space-text-post = {***}]}
% Loading the ``siunitx'' package generates a ``too many math alphabets'' used error.
% See https://tex.stackexchange.com/questions/452682/limit-math-alphabets-created-by-siunitx?noredirect=1&lq=1 and
%https://tex.stackexchange.com/questions/40874/kpfonts-siunitx-and-math-alphabets
% Hence, redefine the (virtually) never used \mathtt command:
\renewcommand{\mathtt}[1]{#1}
% From https://tex.stackexchange.com/questions/213605/siunitx-does-not-detect-semi-bold-font
% ==>
\ExplSyntaxOn\makeatletter
\cs_generate_variant:Nn \tl_if_in:nnTF { noTF }
\cs_set_protected:Npn \__siunitx_detect_font_weight_text: {
	\tl_if_in:noTF { sb bf xb } { \f@series }
	{
		\cs_set:Nn \__siunitx_font_weight: { \boldmath \use:c { \f@series series } }
	}
	{
		\cs_set:Nn \__siunitx_font_weight: { \use:c { \f@series series } }
	}
}
\makeatother\ExplSyntaxOff
% <==

\AtBeginEnvironment{table}{\vspace{-1.2ex}\small}
% Reduces font size in tables slightly and
% reduces excessive white space above tables




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  BIBLIOGRAPHY SETTINGS  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\usepackage[round]{natbib}

\newlength{\bibindent}
\newlength{\bibitemsep}
\newlength{\bibsep}

\setbeamertemplate{bibliography item}{}
\setbeamercolor{bibliography entry author}  {fg=black}
\setbeamercolor{bibliography entry title}   {fg=black}
\setbeamercolor{bibliography entry location}{fg=black}
\setbeamercolor{bibliography entry note}    {fg=black}

\input{0_0_Preamble/Preamble_BibLaTeX_AER}
%\input{0_0_Preamble/Preamble_BibLaTeX_APA}
\bibliography{Library}

\renewcommand{\bibfont}{\scriptsize}

\renewbibmacro*{pageref}{%
	\addperiod
	\iflistundef{pageref}
	{}
	{\color{UBonnGray}%
		\printtext[brackets]{\caps{PDF}~%
			\ifnumgreater{\value{pageref}}{1}
			{pp.}
			{p.}~%
			\printlist[pageref][-\value{listtotal}]{pageref}%
		}%
	}%
}

\setcounter{biburllcpenalty}{7000}
\setcounter{biburlucpenalty}{8000}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  APPENDIX-RELATED SETTINGS  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage{appendixnumberbeamer}
\AtBeginEnvironment{appendix}{%
	\let \insertframenumberorig \insertframenumber
	\renewcommand{\insertframenumber}{Appendix Slide \insertframenumberorig}
	%\let \inserttotalframenumberorig \inserttotalframenumber
	%\renewcommand{\inserttotalframenumber}{A-\inserttotalframenumberorig}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  FOR DEBUGGING ONLY  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage{blindtext}
\blindmathtrue

% An auxiliary command to display the current font settings ==>
\makeatletter
\newcommand{\showfont}{%
	\textit{encoding:} \f@encoding{},
	\textit{family:} \f@family{},
	\textit{series:} \f@series{},
	\textit{shape:} \f@shape{},
	\textit{size:} \f@size{}
}
\makeatother
% <==


==> templates/Preamble_Presentation_IBMPlex.tex <==
% !TeX TXS-program:compile = txs:///pdflatex/
% !BIB program = biber




%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  FUNDAMENTAL SETTINGS  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\serifbodyfont}{0}
% 0: Body is set in sans-serif font
% 1: Body is set in serif font
\newcommand{\serifheadingfont}{1}
% 0: Headings (``structure'') are set in sans-serif font
% 1: Headings (``structure'') are set in serif font

\newcommand{\showsectionnavigation}{0}
% 0: ``Headline'' is disabled.
% 1: ``Headline'' (at the very top of slides) is included and displays all sections of the presentation,
%      with the current section being highlighted.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  FUNDAMENTAL PACKAGES  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage{ifthen}

\usepackage{calc}

\usepackage{tcolorbox}

\usepackage[LY1, LGR, TS1, T1]{fontenc}
% LGR (Greek) is needed to enable the ``sansserif math'' features.
\usepackage[utf8]{inputenc}

\usepackage{tabularx}

\ifxetex
	\usepackage[protrusion=true, expansion=false]{microtype}
\else
	\usepackage[protrusion=true, expansion=false, kerning=true]{microtype}
\fi
% The microtype package enables so-called hanging punctuation. That is, when a punctuation sign like ":", ".", "-", etc. is found at the beginning or end of a line, it is protruded a little into the page margin. This results in "optical margin alignment," because the protrusion makes the margin alignment look straighter.


\definecolor{darkgray}{rgb}{0.4,0.4,0.4}

\usepackage[absolute, overlay]{textpos}
\usepackage{graphicx}
\usepackage{amsmath}
%\usepackage{amsfonts}
%\usepackage{amssymb}
\usepackage{epstopdf}
\DeclareGraphicsRule{.tif}{png}{.png}{`convert #1 `dirname #1`/`basename #1 .tif`.png}

\usepackage[ngerman, american, USenglish]{babel}
% German and US English hyphenation and quotation marks
\selectlanguage{USenglish}
\usepackage[autostyle=true]{csquotes}

\usepackage{multirow}

\usepackage{xcolor}
\usepackage{pgf}%,pgfarrows,pgfnodes,pgfshade}
\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{mindmap, trees, patterns, arrows.meta}

\usepackage{xspace}

% \usepackage{eurosym}

%\usepackage{etoolbox}
%	% Enables manipulating LaTeX commmands via \preto, \appto, \patchcmd, etc.
%	% loaded automatically by beamer
\usepackage{xpatch}
% Enables manipulating LaTeX commmands via \xpatchcmd etc.

\hypersetup{%
	colorlinks, linkcolor=, urlcolor=SpotColor, citecolor=%
}
\urlstyle{same}
\newcommand{\email}[1]{\href{mailto:#1}{\nolinkurl{#1}}}




%%%%%%%%%%%%%%%%%%%%%
%%  FONT SETTINGS  %%
%%%%%%%%%%%%%%%%%%%%%


\input{0_0_Preamble/Preamble_Fonts_IBMPlex}

\ifnum \serifbodyfont=0
	\setbeamerfont{normal text}{family=\sffamily}
	\renewcommand{\familydefault}{\savesffamily}
	\renewcommand{\mddefault}{\savesfmdseries}
	\renewcommand{\bfdefault}{\savesfbfseries}
	\AtBeginDocument{\sffamily}
\else
	\usefonttheme{serif}
	\setbeamerfont{normal text}{family=\rmfamily}
\fi
\ifnum \serifheadingfont=0
	\setbeamerfont{structure}{family=\sffamily, shape=\upshape, series=\bfseries}
\else
	\setbeamerfont{structure}{family=\rmfamily, shape=\upshape, series=\bfseries}
\fi

% Make frame titles and headings bold
\usefonttheme{structurebold}
\usefonttheme{professionalfonts}

\ifnum \serifheadingfont=0
	\setbeamerfont{footline}
		{parent=structure, size=\tiny, series=\mdseries}
\else
	\setbeamerfont{footline}
		{parent=structure, size=\tiny, series=\fontseries{\savermmdseries}}
\fi
\setbeamercolor{footline}
	{fg=SpotColor}

%% Use the bm (= boldmath) package for better support of setting math in bold ==>
%% Prevent the "Too many math fonts used" error:
\newcommand{\bmmax}{0}
\newcommand{\hmmax}{0}
\usepackage{bm}
%% <==

\usepackage{fontawesome}

\usepackage{mathtools}
%\mathtoolsset{centercolon}
% This makes the compilation fail in combination with tikz. See
% https://tex.stackexchange.com/questions/89467/why-does-pdftex-hang-on-this-file.
%% Inspired by https://tex.stackexchange.com/questions/251460/how-to-put-symbols-of-equal-size-on-top-of-each-other
%\newcommand{\succeqq}{%
%	\mathrel{%
%		\vcenter{\offinterlineskip
%			\ialign{##\cr$\succ$\cr\noalign{\kern 1pt}$=$\cr}%
%		}%
%	}%
%}
%\newcommand{\nsucceqq}{\mathrel{\not\succeqq}}
%\newcommand*{\coloneqq}{\mathrel{%
%		\mathrel{%
%			\raisebox{0.15ex}{\scalebox{0.85}{\ensuremath{:}}}\hspace{-0.2pt}%
%		}%
%		=%
%}}

\input{0_0_Preamble/Preamble_Sansserif_math_IBMPlex}

% Allow for fine-grained scaling of font sizes
% ==>
\usepackage{relsize}
\renewcommand\RSpercentTolerance{1}
% Enabling slightly reduced font for CAPS:
\newcommand{\caps}[1]{\textscale{0.96}{\textls[35]{\MakeUppercase{#1}}}}
% <==




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  ADJUSTING THE DESIGN OF THE PRESENTATION  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\linespread{1.1}

\setbeamerfont{title}
	{parent=structure, size=\LARGE}
\ifnum \serifheadingfont=0
	\setbeamerfont{subtitle}
		{parent=structure, size=\Large, series=\mdseries}
\else
	\setbeamerfont{subtitle}
		{parent=structure, size=\Large, series=\fontseries{\savermmdseries}}
\fi
\setbeamerfont{frametitle}
	{parent=structure, size=\large}

% For convenience, let the ``paperheight'' of the slides be identical,
% no matter what the aspect ratio of the slides ==>
\makeatletter
% 4:3 aspect ratio:
\@ifclasswith{beamer}{aspectratio=43}{%
	\beamer@paperwidth 12.00cm%
	\beamer@paperheight 9.00cm%
	\setbeamerfont{title}
		{parent=structure, size*={16}{20}}
	\setbeamerfont{subtitle}
		{parent=structure, size*={13.5}{17}}
	\setbeamerfont{frametitle}
		{parent=structure, size*={11}{14}}
}{}
%% 14:9 aspect ratio: Nothing needs to be changed
%\@ifclasswith{beamer}{aspectratio=149}{%
%	\beamer@paperwidth 14.00cm%
%	\beamer@paperheight 9.00cm%
%}{}
%% 16:9 aspect ratio: Nothing needs to be changed
%\@ifclasswith{beamer}{aspectratio=169}{%
%	\beamer@paperwidth 16.00cm%
%	\beamer@paperheight 9.00cm%
%}{}
% 16:10 aspect ratio:
\@ifclasswith{beamer}{aspectratio=1610}{%
	\beamer@paperwidth 14.40cm%
	\beamer@paperheight 9.00cm%
}{}
\makeatother
% <==

% Margins ==>
\newcommand{\margintop}{12.5pt}
\newcommand{\marginleft}{17.5pt}
\newcommand{\marginright}{\marginleft}
\setbeamersize{text margin left=\marginleft}
\setbeamersize{text margin right=\marginright}
\setlength{\textwidth}{\paperwidth-\marginleft-\marginright}
% <==

\setlength{\parskip}{\medskipamount}
% Inserts some space between paragraphs

% Enable hyphenation on Beamer slides:
\usepackage{ragged2e}
\let \raggedright \RaggedRight
\sloppy
\hyphenpenalty=500

\setbeamerfont{alerted text}{series=\bfseries}

\definecolor{OSEBlue}	  {RGB}{  0,  76, 141}
%\definecolor{OSEBlueLight}{RGB}{ 48, 188, 237}
\definecolor{OSEBlueLight}{RGB}{ 51, 153, 204}
\definecolor{UBonnBlue}   {RGB}{  7,  82, 154}
\definecolor{UBonnYellow} {RGB}{234, 185,  12}
\definecolor{UBonnGray}   {RGB}{144, 144, 133}
\definecolor{darkgray}    {RGB}{102, 102, 102}
\definecolor{darkred}     {RGB}{191,   0,   0}
\definecolor{neutralgreen}{RGB}{ 28, 166,   0}

\colorlet{SpotColor}   {OSEBlue}
\colorlet{AlertColor}  {OSEBlue}
%\colorlet{ExampleColor}{neutralgreen}
\colorlet{ExampleColor}{OSEBlueLight}
\definecolor{darkgrey}{gray}{0.65}
\definecolor{lightblue}{rgb}{0.8,0.85,1}
\definecolor{darkgray}{rgb}{0.4,0.4,0.4}
\definecolor{darkblue}{rgb}{0,.35,.62}
\definecolor{lightblue}{rgb}{0.8,0.85,1}
\definecolor{lightgrey}{gray}{0.1}	%Farben mischen
\definecolor{Gray}{gray}{0.9}
\definecolor{mplorange}{HTML}{FF7F0E}
\definecolor{mplred}{HTML}{D62728}
\definecolor{mplblue}{HTML}{1F77B4}
\definecolor{mplgreen}{HTML}{2CA02C}
\definecolor{tabblue}{RGB}{31,119,180}  % usage: blue-collar occupation
\definecolor{taborange}{RGB}{255, 127, 14}  % usage: school
\definecolor{tabgreen}{RGB}{44, 160, 44}  % usage: home
\definecolor{tabred}{RGB}{214, 39, 40}  % usage: white-collar occupation
\definecolor{tabpurple}{RGB}{148, 103, 189}  % usage: military
\definecolor{tabbrown}{RGB}{140, 86, 75}
\definecolor{tabrose}{RGB}{227, 119, 194}
\definecolor{tabgrey}{RGB}{127, 127, 127}
\definecolor{tablime}{RGB}{188, 189, 34}
\definecolor{tabcyan}{RGB}{23, 190, 207}
\setbeamercolor{structure}{fg=SpotColor}
\setbeamercolor{alerted text}{fg=AlertColor}
\setbeamercolor{author in head/foot}{fg=white, bg=SpotColor}
\setbeamercolor{button}{bg=SpotColor,fg=white}
\setbeamercolor{headline}{bg=SpotColor,fg=white}
\setbeamercolor{headlinecover}{bg=white,fg=white}

\newcommand{\highlight}[1]{\textcolor{SpotColor}{#1}}
\newcommand{\heading}[1]{%
	\par%
	\textbf{\usebeamerfont{structure}\usebeamercolor[fg]{frametitle}#1}%
	\par%
}

%\renewcommand{\alert}[1]{\highlight{\textbf{#1}}}

\newlength{\rulelength}
\setlength{\rulelength}{\paperwidth - \marginleft - \marginright}
\newcommand{\sliderule}{%
	\textcolor{SpotColor}{\rule{\rulelength}{.35pt}}%
}

% Remove navigation symbols from the slide footer
\beamertemplatenavigationsymbolsempty

% Adjust layout of frametitle
% ==>
\setbeamertemplate{frametitle}{%
	\vspace{\margintop}\vspace{-5pt}%
	{\large\usebeamercolor{frametitle}\usebeamerfont{frametitle}\insertframetitle\\[-1.2ex]}%
	\sliderule%
}
% <==

\newlength{\navigationwidth}
\BeforeBeginEnvironment{frame}{%
	% Add a slide number (and [short]title) to the footer of each slide
	% ==>
	\setbeamertemplate{footline}{\vskip-15pt%
		\hspace{\marginleft}%
		\sliderule \vspace{1.1ex} \linebreak
		\mbox{\hspace{\marginleft}}%
		\insertshortauthor: \enquote{\insertshorttitle}
		\hfill%
		\textbf{\insertframenumber/\inserttotalframenumber}%
		\hspace{\marginright}%
		\vspace{12pt}%
	}%
	% <==
	% Outline with current section highlighted in the ``headline'' ==>
	\ifnum \showsectionnavigation=0
	\setbeamertemplate{headline}{}
	\else
	\setbeamertemplate{headline}{%
		\hspace{\marginleft}%
		\begin{beamercolorbox}[wd=\linewidth, ht=5pt, dp=2pt]{headline}%
			\insertsectionnavigationhorizontal{\linewidth}{\hspace{0.04\linewidth}}{\hspace{0.04\linewidth}}%
		\end{beamercolorbox}%
		\newline
		\begin{beamercolorbox}[wd=\paperwidth, ht=15pt, dp=0pt]{headlinecover}%
			% Adds a white bar to cover stuff that protrudes from the above color box.
		\end{beamercolorbox}%
	}
	\setlength{\fboxrule}{0.25pt}\setlength{\fboxsep}{7.5pt}%
	\setbeamertemplate{section in head/foot}{%
		\settowidth{\navigationwidth}{\bfseries\insertsectionhead}%
		\fcolorbox{SpotColor!25}{SpotColor}{%
			\makebox[\navigationwidth]{\color{white}\bfseries\insertsectionhead}%
		}%
	}
	\setbeamertemplate{section in head/foot shaded}{%
		\settowidth{\navigationwidth}{\bfseries\insertsectionhead}%
		\fcolorbox{SpotColor}{SpotColor}{%
			\makebox[\navigationwidth]{\color{white}\mdseries\insertsectionhead}%
		}
	}
	\fi
	% <==
}

% See https://tex.stackexchange.com/questions/427257/how-to-remove-footer-for-specific-type-of-slides-frames
% ==>
\makeatletter
\define@key{beamerframe}{standout}[true]{%
	\setbeamertemplate{footline}{\vskip-15pt%
		\hspace{\marginleft}%
		\sliderule \vspace{1.1ex} \linebreak
		\mbox{\hspace{\marginleft}}%
		\textmd{\phantom{\insertshortauthor: \enquote{\insertshorttitle}}}
		\hfill%
		\phantom{\insertframenumber/\inserttotalframenumber}%
		\hspace{\marginright}%
		\vspace{15pt}%
	}%
	\setbeamertemplate{headline}{}%
}
\makeatother
% <==

\frenchspacing  % Prevent increased whitespace after periods and colons

\setbeamertemplate{button}{%
	\tikz
	\node[
	inner xsep=3pt,
	inner ysep=2pt,
	draw=structure!100,
	fill=structure!100,
	rounded corners=1.5pt
	]{\raisebox{1.5pt}{\usebeamerfont{structure}\insertbuttontext}};%
}

%\renewcommand{\texteuro}{\fontencoding{TS1}\selectfont\char"BF\fontencoding{T1}\selectfont}
%\newcommand{\euro}{\texteuro}

% Adding framenumbers automatically to the frametitles
\newcommand{\pageinsection}{\number\numexpr\insertpagenumber-\insertsectionstartpage+1}
% From https://tex.stackexchange.com/questions/308343/how-to-create-mini-sections-mini-subsections-and-mini-frames-in-beamer-presenta
% ==>
%\usepackage{etoolbox}  % Automatically loaded by beamer
\makeatletter
\newcount\beamer@sectionstartframe
\beamer@sectionstartframe=1
\apptocmd{\beamer@section}{%
	\addtocontents{nav}{\protect\headcommand{%
			\protect\beamer@sectionframes{\the\beamer@sectionstartframe}{\the\c@framenumber}}}%
}{}{}
\apptocmd{\beamer@section}{%
	\beamer@sectionstartframe=\c@framenumber\advance\beamer@sectionstartframe by1\relax%
}{}{}
\AtEndDocument{%
	\immediate\write\@auxout{\string\@writefile{nav}%
		{\noexpand\headcommand{\noexpand\beamer@sectionframes{\the\beamer@sectionstartframe}{\the\c@framenumber}}}}%
}{}{}
\def\beamer@startframeofsection{1}
\def\beamer@endframeofsection{1}
\def\beamer@sectionframes#1#2{%
	\ifnum\c@framenumber<#1%
	\else%
	\ifnum\c@framenumber>#2%
	\else%
	\gdef\beamer@startframeofsection{#1}%
	\gdef\beamer@endframeofsection{#2}%
	\fi%
	\fi%
}
\newcommand\insertsectionstartframe{\beamer@startframeofsection}
\newcommand\insertsectionendframe{\beamer@endframeofsection}
\makeatother
% <==
\newcommand{\frameinsection}{\number\numexpr\insertframenumber-\insertsectionstartframe+1}
% https://tex.stackexchange.com/questions/228684/two-counters-for-beamer-presentations
%\newcommand{\titleprefix}{\insertsection~{\pageinsection}}
\newcommand{\titleprefix}{\insertsection~{\frameinsection}}
% <==

% Continuation counter for frames with the ``allowframebreaks'' option.
% ==>
%% Inspired by https://tex.stackexchange.com/questions/275044/how-do-i-insert-the-total-continuation-count-in-the-allowframbreaks-frame-title:
%\newcounter{totalcontinuationcount}
%\makeatletter
%\setbeamertemplate{frametitle continuation}{%
%	\setcounter{totalcontinuationcount}{\beamer@endpageofframe}%
%	\addtocounter{totalcontinuationcount}{1}%
%	\addtocounter{totalcontinuationcount}{-\beamer@startpageofframe}%
%	\ifnum \value{totalcontinuationcount} > 1
%		\textmd{(\insertcontinuationcount/\arabic{totalcontinuationcount})}%
%	\fi
%}
%\makeatother
% More elegant version based on https://github.com/josephwright/beamer/issues/423#issuecomment-456494500:
\makeatletter
\defbeamertemplate*{frametitle continuation}{only if multiple}{%
	\ifnum \numexpr\beamer@endpageofframe+1-\beamer@startpageofframe\relax > 1
	\textmd{(%
		\insertcontinuationcount/%
		\the\numexpr\beamer@endpageofframe+1-\beamer@startpageofframe%
		)}%
	\fi%
}
\makeatother
% <==




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  LAYOUT OF THE TITLE SLIDE  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Make the title page left-aligned
% ==>
%\setbeamertemplate{title page}[default][left]

% \setbeamerfont{title} and \setbeamerfont{subtitle} already executed above!
\setbeamerfont{author}
	{parent=normal text, size=\large, series=\mdseries, shape=\upshape}
\setbeamercolor{author}
	{parent=normal text}
\setbeamerfont{institute}
	{parent=normal text, size=\small, series=\mdseries, shape=\itshape}
\setbeamercolor{institute}
	{parent=normal text}
\ifnum \serifheadingfont=0
	\setbeamerfont{date}
	{parent=structure, size=\normalsize, series=\bfseries}
\else
	\setbeamerfont{date}
	{parent=structure, size=\normalsize, series=\fontseries{semibold}}
\fi
\setbeamercolor{date}
	{parent=normal text}

\makeatletter
\setbeamertemplate{title page}{
	\begin{minipage}[c][6.75cm]{\textwidth}%
		\raggedright%
		\ifx\inserttitlegraphic\@empty\else%
		\inserttitlegraphic%
		\fi
		\vfill
		\begingroup
		\ifx\inserttitle\@empty\else%
		\usebeamerfont{title}\usebeamercolor[fg]{title}\inserttitle\par%
		\fi
		\ifx\insertsubtitle\@empty\else%
		\medskip
		\usebeamerfont{subtitle}\usebeamercolor[fg]{subtitle}\insertsubtitle\par%
		\fi
		\ifx\beamer@shortauthor\@empty\else%
		\vspace{\fill}
		\usebeamerfont{author}\usebeamercolor[fg]{author}\insertauthor\par%
		\fi
		\ifx\insertinstitute\@empty\else%
		\vspace{\fill}
		\usebeamerfont{institute}\usebeamercolor[fg]{institute}\insertinstitute\par%
		\fi
		\ifx\insertdate\@empty\else%
		\vspace{\fill}
		\usebeamerfont{date}\usebeamercolor[fg]{date}\insertdate%
		\fi
		\endgroup
		\vfill
		\vspace{0cm}  % For the \vfill to actually have an effect
	\end{minipage}%
}
\makeatother
% <==

\makeatletter
\renewcommand{\beamer@insttitle}[1]{\highlight{\textsuperscript{\kern.75pt \textit{#1}}}}
\renewcommand{\beamer@instinst}[1]{\beamer@insttitle{#1}\ignorespaces}
\renewcommand{\beamer@andinst}{\\[0.33\baselineskip]}
\makeatother




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  LAYOUT OF THE TABLE OF CONTENTS  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\useinnertheme{circles}
\setbeamertemplate{section in toc}{%
	\leavevmode\leftskip=3.3ex%
	\llap{%
		\usebeamerfont*{section number projected}%
		\usebeamercolor{section number projected}%
		\begin{pgfpicture}{-1ex}{0ex}{1ex}{2ex}
			\color{bg}
			\pgfpathcircle{\pgfpoint{0pt}{.75ex}}{1.2ex}
			\pgfusepath{fill}
			\pgftext[base]{\color{fg}\raisebox{0.07ex}{%
					% \addfontfeatures{Numbers={Lining, Monospaced}}%
					\usebeamerfont{structure}%
					\small\inserttocsectionnumber}%
			}
		\end{pgfpicture}\kern1.5ex%
	}%
	\usebeamerfont{normal text}%
	\inserttocsection\par%
}
\setbeamertemplate{subsection in toc}{%
	\leavevmode\leftskip=2em$\bullet$\hskip1em\inserttocsubsection\par%
}

\makeatletter
\patchcmd{\beamer@sectionintoc}
{\vfill}
{\medskip}
{}
{}
\makeatother




%%%%%%%%%%%%%%
%%  BLOCKS  %%
%%%%%%%%%%%%%%


% Put border around block, exampleblock, and alertblock
% ==>

\usepackage{mdframed}
\usepackage{changepage}

\newlength{\blockinnermargin}
\setlength{\blockinnermargin}{4pt}

\newcommand{\framedblockcolor}{SpotColor}  % This allows us to change the color mid-presentation
\newcommand{\PutBorderAroundBlock}[2]{
	\renewcommand{\framedblockcolor}{#2}%
	\setbeamercolor*{block title}{fg=white, bg=\framedblockcolor}%
	\setbeamercolor*{block body} {fg=black, bg=}%
	\addtobeamertemplate{block begin}{%
		\setbeamercolor*{item}{fg=\framedblockcolor}%
		\begin{mdframed}[linecolor=\framedblockcolor, linewidth=0.35pt, leftmargin=0pt, innerleftmargin=0.375em, innerrightmargin=0.375em, innertopmargin=-0.01ex, innerbottommargin=4pt]%
			\let \insertblocktitleorig \insertblocktitle%
			\renewcommand{\insertblocktitle}{%
				\RaggedRight%
				\leftskip=\blockinnermargin%
				\rightskip=\blockinnermargin%
				\insertblocktitleorig\strut\vspace{-1.5pt}%
					% \strut\vspace{-1.5pt} so that all single-line block titles have identical hight
			}%
	}{%
		\renewcommand{\insertblocktitle}{\insertblocktitleorig}%
		\begin{adjustwidth}{\blockinnermargin}{\blockinnermargin}%
			\RaggedRight%
	}%
	\addtobeamertemplate{block end}{%
		\end{adjustwidth}%
	}{%
		\end{mdframed}%
	}%
}
\PutBorderAroundBlock{}{SpotColor}  % Default color of blocks is SpotColor

\newcommand{\PutBorderAroundBlockExAlert}[2]{%
	\def\temp{#1}%
	\ifx\temp\empty
		\def\blocktype{block }     % Trailing space is crucial!
	\else
		\def\temp{ #1}
		\def\blocktype{block #1 }  % Trailing space is crucial!
	\fi
	\setbeamercolor*{block title\temp}{fg=white, bg=#2}
	\setbeamercolor*{block body\temp} {fg=black, bg=}
	\addtobeamertemplate{\blocktype begin}{%
		\begin{mdframed}[linecolor=#2, linewidth=0.35pt, leftmargin=0pt, innerleftmargin=0.375em, innerrightmargin=0.375em, innertopmargin=-0.01ex, innerbottommargin=4pt]%
			\let \insertblocktitleorig \insertblocktitle%
			\renewcommand{\insertblocktitle}{%
				\RaggedRight%
				\leftskip=\blockinnermargin%
				\rightskip=\blockinnermargin%
				\insertblocktitleorig\strut\vspace{-1.5pt}%
					% \strut\vspace{-1.5pt} so that all single-line block titles have identical hight
			}%
	}{%
		\renewcommand{\insertblocktitle}{\insertblocktitleorig}%
		\begin{adjustwidth}{\blockinnermargin}{\blockinnermargin}%
			\RaggedRight%
	}%
	\addtobeamertemplate{\blocktype end}{%
		\end{adjustwidth}%
	}{%
		\end{mdframed}%
	}%
}
\PutBorderAroundBlockExAlert{example}{ExampleColor}
\PutBorderAroundBlockExAlert{alerted}{AlertColor}

% <==

% Style definition, theorem, lemma, corollary, and proof with out border
% ==>

% Inspired by https://github.com/schnorr/infufrgs/blob/master/slides/beamerthemeInf.sty
\setbeamercolor{theorem title}{fg=SpotColor}
\setbeamerfont{theorem title}{parent=structure}
\setbeamercolor{theorem body}{fg=black}
\setbeamerfont{theorem body}{parent=normal text, shape=\itshape, series=\mdseries}
% Body of theorem, lemma, and corollary are italicized
\AtBeginEnvironment{definition}{%
	\setbeamerfont{theorem body}{parent=normal text, shape=\upshape, series=\mdseries}
	% Body of definition is typeset in upright font
}

\setbeamertemplate{theorem begin}{%
	\usebeamerfont{theorem title}%
	\usebeamercolor[fg]{theorem title}%
	\inserttheoremname%~\inserttheoremnumber%
	\ifx\inserttheoremaddition\empty\else\ (\inserttheoremaddition)\fi%
	%\inserttheorempunctuation\hspace{1ex}%
	\\[\smallskipamount]
	\usebeamerfont{theorem body}%
	\usebeamercolor[fg]{theorem body}%
}
\setbeamertemplate{theorem end}{}

\setbeamercolor{proof title}{fg=SpotColor}
\setbeamerfont {proof title}{parent=structure}
\setbeamercolor{proof body} {fg=black}
\setbeamerfont {proof body} {parent=normal text, shape=\upshape, series=\mdseries}
% Remove period after ``Proof''
% See https://tex.stackexchange.com/questions/31354/how-to-remove-the-in-the-proof-environment
% -->
\makeatletter
\let\@addpunct\@gobble
\makeatother
% <--
\renewcommand{\qedsymbol}{\small\textcolor{SpotColor}{$\blacksquare$}}
\setbeamertemplate{proof begin}{%
	\usebeamerfont{proof title}%
	\usebeamercolor[fg]{theorem title}%
	\insertproofname\\[\smallskipamount]
	\usebeamerfont{proof body}%
	\usebeamercolor[fg]{proof body}%
}
\setbeamertemplate{proof end}{}

% <==




%%%%%%%%%%%%%
%%  LISTS  %%
%%%%%%%%%%%%%


\AtBeginEnvironment{itemize}{%
	\vspace{-\parskip}%
	\setlength{\labelsep}{0.55em}%
	\setlength{\labelwidth}{\widthof{9.}}%
}
\AtBeginEnvironment{enumerate}{%
	\vspace{-\parskip}%
	\setlength{\labelsep}{0.5em}%
	\setlength{\labelwidth}{\widthof{9.}}%
}

% Adjust spacing of lists ==>
% Unfortunately, the ``enumitem'' package is incompatible with the ``beamer'' class.
% Hence, we need to adjust left margins etc. manually:
\setlength{\leftmargini}{\widthof{9.}+\labelsep}
\setlength{\leftmarginii}{\widthof{g.}+\labelsep}
\setlength{\leftmarginiii}{\widthof{iii.}+\labelsep}
%\setlength{\rightmargin}{0in}
%\setlength{\itemindent}{0in}
%\usepackage{enumitem}
%\setlist[enumerate, 1]{
%	leftmargin=-\parindent, listparindent=\parindent, labelsep=0.42\parindent, itemsep=\smallskipamount, parsep=0pt
%}
%
%\setlist[itemize, 1]{
%	leftmargin=0pt, listparindent=\parindent, labelsep=0.75em, itemsep=\smallskipamount, parsep=0pt, topsep=1.2ex, label=\usebeamerfont*{itemize item}	\usebeamercolor[fg]{itemize item} \usebeamertemplate{itemize item}, before={\RaggedRight \hyphenpenalty=1000}
%}
%\setlist[itemize, 2]{
%	leftmargin=1.2em, listparindent=\parindent, labelsep=0.6em, itemsep=\smallskipamount, parsep=0pt, topsep=0.6ex, label=\usebeamercolor[fg]{itemize item} --, before={\RaggedRight \hyphenpenalty=1000}
%}
% <==

% ``Medium'' as the bold series:
%\makeatletter
%\def\bfseries@sf{mb}
%\makeatother

%\useinnertheme{circles}

\setbeamertemplate{enumerate items}
[default]
\setbeamertemplate{enumerate subitem}
{\alph{enumii}.}
\setbeamertemplate{enumerate subsubitem}
{\roman{enumiii}.}

\setbeamertemplate{itemize item}
{\raisebox{-0.5pt}{\scalebox{0.95}{\textrm{\textbf{\textbullet}}}}\hspace{-0.06em}}
\setbeamertemplate{itemize subitem}
{\usebeamerfont{normal text}--\hspace{0.15em}}
\setbeamertemplate{itemize subsubitem}
{\raisebox{1.5pt}{\tiny$\blacktriangleright$}\hspace{0.15em}}

\setbeamerfont*{itemize/enumerate body}{size=\normalsize}
\setbeamerfont*{itemize/enumerate subbody}{parent=itemize/enumerate body}
\setbeamerfont*{itemize/enumerate subsubbody}{parent=itemize/enumerate body}

\renewenvironment{quote}{%
	\list{}{\leftmargin\leftmarginii \rightmargin\leftmarginii}%
	\RaggedLeft
	\itshape%
	\item\relax%
}
{\endlist}




%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  FIGURES AND TABLES  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%


\setbeamertemplate{caption}[numbered]
\setbeamertemplate{caption label separator}{. }
\usepackage[justification=centering]{caption}
\ifnum \serifbodyfont=0
	\captionsetup{font={sf, small}}
\else
	\captionsetup{font={rm, small}}
\fi
\ifnum \serifheadingfont=0
	\captionsetup{labelfont={sf, small, bf, color=SpotColor}}
\else
	\captionsetup{labelfont={rm, small, bf, color=SpotColor}}
\fi

\usepackage{tabularx}	% Provides environment tabularx to adjust width of tables
% \usepackage{tabulary}	% For some reason, tabulary doesn't obey the width argument ...
% Emulate the "tabulary" column types:
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{J}{>{\arraybackslash}X}
\newcolumntype{L}{>{\RaggedRight\arraybackslash}X}
\newcolumntype{R}{>{\RaggedLeft\arraybackslash}X}
% \usepackage[flushleft]{threeparttable}	% Provides the tablenotes environment


% Packages for creating better-looking tables
\usepackage{booktabs}
\setlength{\cmidrulewidth}{.35pt}
\setlength{\lightrulewidth}{.35pt}
\setlength{\heavyrulewidth}{.70pt}
\setlength{\abovetopsep}{-8pt}
\addtolength{\aboverulesep}{1pt}	% Make tables a little more spacious
\addtolength{\belowrulesep}{1pt}
% \setlength{\belowbottomsep}{-2pt}
\usepackage{colortbl} % e.g., for colored rules
\arrayrulecolor{SpotColor} % Color all table rules blue

\usepackage{siunitx}
% Allows, among others, for alignment of decimal numbers in tables at the decimal point.
\sisetup{
	detect-all,
	round-integer-to-decimal = true,
	group-digits             = true,
	group-minimum-digits     = 5,
	group-separator          = {\kern 1pt},
	table-align-text-pre     = false,
	table-align-text-post    = false,
	input-signs              = + -,
	input-symbols            = {*} {**} {***} \sigstar,
	input-open-uncertainty 	 = ,
	input-close-uncertainty  = ,
	retain-explicit-plus
}
\newcolumntype{T}[1]
{@{}S[table-format = #1, table-space-text-pre = {***}, table-space-text-post = {***}]}
% Loading the ``siunitx'' package generates a ``too many math alphabets'' used error.
% See https://tex.stackexchange.com/questions/452682/limit-math-alphabets-created-by-siunitx?noredirect=1&lq=1 and
%https://tex.stackexchange.com/questions/40874/kpfonts-siunitx-and-math-alphabets
% Hence, redefine the (virtually) never used \mathtt command:
\renewcommand{\mathtt}[1]{#1}
% From https://tex.stackexchange.com/questions/213605/siunitx-does-not-detect-semi-bold-font
% ==>
\ExplSyntaxOn\makeatletter
\cs_generate_variant:Nn \tl_if_in:nnTF { noTF }
\cs_set_protected:Npn \__siunitx_detect_font_weight_text: {
	\tl_if_in:noTF { sb bf xb } { \f@series }
	{
		\cs_set:Nn \__siunitx_font_weight: { \boldmath \use:c { \f@series series } }
	}
	{
		\cs_set:Nn \__siunitx_font_weight: { \use:c { \f@series series } }
	}
}
\makeatother\ExplSyntaxOff
% <==

\AtBeginEnvironment{table}{\vspace{-1.2ex}\small}
% Reduces font size in tables slightly and
% reduces excessive white space above tables




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  BIBLIOGRAPHY SETTINGS  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\usepackage[round]{natbib}

\newlength{\bibindent}
\newlength{\bibitemsep}
\newlength{\bibsep}

\input{0_0_Preamble/Preamble_BibLaTeX_AER}
\bibliography{Library}

\renewcommand{\bibfont}{\scriptsize}

\setbeamertemplate{bibliography item}{}
\setbeamercolor{bibliography entry author}  {fg=black}
\setbeamercolor{bibliography entry title}   {fg=black}
\setbeamercolor{bibliography entry location}{fg=black}
\setbeamercolor{bibliography entry note}    {fg=black}

\renewbibmacro*{pageref}{%
	\addperiod
	\iflistundef{pageref}
	{}
	{\color{UBonnGray}%
		\printtext[brackets]{\caps{PDF}~%
			\ifnumgreater{\value{pageref}}{1}
			{pp.}
			{p.}~%
			\printlist[pageref][-\value{listtotal}]{pageref}%
		}%
	}%
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  APPENDIX-RELATED SETTINGS  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage{appendixnumberbeamer}
\AtBeginEnvironment{appendix}{%
	\let \insertframenumberorig \insertframenumber
	\renewcommand{\insertframenumber}{Appendix Slide \insertframenumberorig}
	%\let \inserttotalframenumberorig \inserttotalframenumber
	%\renewcommand{\inserttotalframenumber}{A-\inserttotalframenumberorig}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  FOR DEBUGGING ONLY  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage{blindtext}
\blindmathtrue

% An auxiliary command to display the current font settings ==>
\makeatletter
\newcommand{\showfont}{%
	\textit{encoding:} \f@encoding{},
	\textit{family:} \f@family{},
	\textit{series:} \f@series{},
	\textit{shape:} \f@shape{},
	\textit{size:} \f@size{}
}
\newcommand{\showfamily}{\f@family{}}
\makeatother
% <==


==> templates/Preamble_Sansserif_math_IBMPlex.tex <==
% !TeX TXS-program:compile = txs:///pdflatex/
% !TeX program = pdflatex




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  SANS-SERIF MATH IN SANS-SERIF ENVIRONMENT  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% See https://tex.stackexchange.com/questions/41497/how-to-typeset-some-text-including-math-content-in-sans-serif
% See https://tex.stackexchange.com/questions/33165/make-mathfont-respect-the-surrounding-family

% Necessary for use of kpfonts
% ==>
\makeatletter
\newif\ifkp@upRm
\newif\ifkp@osm
\newif\ifkp@vosm
\makeatother
% <==

\DeclareMathVersion{normalup}
\DeclareMathVersion{boldup}
\DeclareMathVersion{sans}

%\DeclareSymbolFont{operators}{OT1}{ntxtlf}{m}{n}

%\SetSymbolFont{operators}{normal}{OT1}{ntxtlf}{m}{n}
%\SetSymbolFont{operators}{bold}  {OT1}{ntxtlf}{bx}{n}

%\SetSymbolFont{operators}{sans}{OT1}{jkpss}{m}{n}
%	% From http://mirrors.ctan.org/fonts/kpfonts/latex/kpfonts.sty
%\SetSymbolFont{operators}   {sans}{OT1}{ntxtlf}{m}{n}
%\SetSymbolFont{letters}     {sans}{OML}{jkpss}{m}{it}
% From http://mirrors.ctan.org/fonts/kpfonts/latex/kpfonts.sty
%\SetSymbolFont{letters}     {sans}{OML}{cmbrm}{m}{it}
%\SetSymbolFont{symbols}     {sans}{OMS}{cmbrs}{m}{n}
%\SetSymbolFont{symbols}     {sans}{OMS}{jkp}  {m}{n}
% From http://mirrors.ctan.org/fonts/kpfonts/latex/kpfonts.sty
%\SetSymbolFont{symbols}{sans}{LMS}{ntxsy}{m}{n}
	% From http://mirrors.ctan.org/fonts/newtx/tex/newtxmath.sty
%\DeclareSymbolFont{extrasymbols}  {OMS}{cmbrs}{m}{n}
%\SetSymbolFont{extrasymbols}{sans}{OMS}{cmbrs}{m}{n}
% Some symbols (e.g., \prime) look weird in kpfonts.
% This provides the option to replace them by symbols from mathdesign-charter.

\SetMathAlphabet{\mathit} {normal}{T1}{\savermfamily}{\savermmdseries}{it}
\SetMathAlphabet{\mathit} {bold}  {T1}{\savermfamily}{\savermbfseries}{it}

\SetMathAlphabet{\mathit} {sans}{T1}{\savesffamily}{\savesfmdseries}{it}
\SetMathAlphabet{\mathbf} {sans}{T1}{\savesffamily}{\savesfbfseries}{n}
\SetMathAlphabet{\mathtt} {sans}{OT1}{cmtl}{m}{n}
\SetMathAlphabet{\mathcal}{sans}{LMS}{ntxsy}{m}{n}
% See https://tex.stackexchange.com/questions/231583/import-mathcal-symbols-from-txfonts
%\SetSymbolFont{largesymbols}{sans}{OMX}{jkpss}{m}{n}
%	% From http://mirrors.ctan.org/fonts/kpfonts/latex/kpfonts.sty
%\SetSymbolFont{largesymbols} {sans}{OMX}{mdbch}{m}{n}
% Using symbols like \int, \left(, etc. from mathdesign-charter because they look better than the ones included in kpfonts
% Using symbols like \int, \left(, etc. from newtxmath:
%\DeclareSymbolFont{largesymbols}{LMX}{ntxexx}{m}{n}
\SetSymbolFont{largesymbols}{sans}{LMX}{ntxexx}{m}{n}

\DeclareMathVersion{sansup}
%\SetSymbolFont{letters}  {sansup}{OML}{jkpss}{m}{it}
%\SetSymbolFont{symbols}  {sansup}{OMS}{jkp}  {m}{n}
%\SetSymbolFont{symbols}{sansup}{LMS}{ntxsy}{m}{n}
	% From http://mirrors.ctan.org/fonts/newtx/tex/newtxmath.sty

\DeclareMathVersion{boldsans}
%\SetSymbolFont{operators}{boldsans}{OT1}{jkpss}{b}{n}
%	% From http://mirrors.ctan.org/fonts/kpfonts/latex/kpfonts.sty
%\SetSymbolFont{operators}{boldsans}{OT1}{ntxtlf}{bx}{n}
%\SetSymbolFont{letters}  {boldsans}{OML}{jkpss}{bx}{it}
% From http://mirrors.ctan.org/fonts/kpfonts/latex/kpfonts.sty
%\SetSymbolFont{letters}  {boldsans}{OML}{mdbch}{bx}{it}
%\SetSymbolFont{letters}{boldsans}{OML}{cmbrm}{b}{it}
%\SetSymbolFont{symbols}  {boldsans}{OMS}{jkp}  {bx}{n}
% From http://mirrors.ctan.org/fonts/kpfonts/latex/kpfonts.sty
\SetSymbolFont{letters} {boldsans}{OML}{nxlmi} {b}{it}
\SetSymbolFont{lettersA}{boldsans}{U}  {ntxmia}{b}{it}
\SetSymbolFont{symbols} {boldsans}{LMS}{ntxsy} {b}{n}
	% From http://mirrors.ctan.org/fonts/newtx/tex/newtxmath.sty
%\SetMathAlphabet{\mathrm}{boldsans}{OT1}{\savesffamily}{\savesfbfseries}{n}
\SetMathAlphabet{\mathit} {boldsans}{T1}{\savesffamily}{\savesfbfseries}{it}
\SetMathAlphabet{\mathtt} {boldsans}{T1}{cmtl}{b}{n}
\SetMathAlphabet{\mathcal}{boldsans}{LMS}{ntxsy}{b}{n}
%\SetSymbolFont{largesymbols}{boldsans}{OMX}{jkpss}{bx}{n}
%	% From http://mirrors.ctan.org/fonts/kpfonts/latex/kpfonts.sty
%\SetSymbolFont{largesymbols}{boldsans}{OMX}{mdbch}{bx}{n}
% Using symbols like \int, \left(, etc. from mathdesign-charter because they look better than the ones included in kpfonts
% Using symbols like \int, \left(, etc. from newtxmath:
\SetSymbolFont{largesymbols}{boldsans}{LMX}{ntxexx}{b}{n}

\DeclareMathVersion{boldsansup}
%\SetSymbolFont{letters}{boldsansup}{OML}{jkpss}{bx}{it}
%\SetSymbolFont{symbols}{boldsansup}{OMS}{jkp}  {bx}{n}
\SetSymbolFont{letters} {boldsans}  {OML}{nxlmi} {b}{it}
\SetSymbolFont{lettersA}{boldsansup}{U}  {ntxmia}{b}{it}
\SetSymbolFont{symbols} {boldsansup}{LMS}{ntxsy} {b}{n}
\SetSymbolFont{lettersA}{normalup}  {U}  {ntxmia}{m}{it}
\SetSymbolFont{lettersA}{boldup}    {U}  {ntxmia}{b}{it}
	% From http://mirrors.ctan.org/fonts/newtx/tex/newtxmath.sty
	% Upright Greek characters are taken from the lettersA font.

% Using glyphs for math mode from the custom sansserif font
\DeclareSymbolFont{uprightglyphs}{T1}{\savermfamily}{\savermmdseries}{n}
%\DeclareSymbolFontAlphabet{\mathrm}{uprightglyphs}
%\SetMathAlphabet{\mathrm}{normal}{OT1}{\savermfamily}{\savermmdseries}{n}
\SetSymbolFont{uprightglyphs}{normal}    {T1}{\savermfamily}{\savermmdseries}{n}
\SetSymbolFont{uprightglyphs}{normalup}  {T1}{\savermfamily}{\savermmdseries}{n}
\SetSymbolFont{uprightglyphs}{bold}      {T1}{\savermfamily}{\savermbfseries}{n}
\SetSymbolFont{uprightglyphs}{boldup}    {T1}{\savermfamily}{\savermbfseries}{n}
\SetSymbolFont{uprightglyphs}{sans}      {T1}{\savesffamily}{\savesfmdseries}{n}
\SetSymbolFont{uprightglyphs}{sansup}    {T1}{\savesffamily}{\savesfmdseries}{n}
\SetSymbolFont{uprightglyphs}{boldsans}  {T1}{\savesffamily}{\savesfbfseries}{n}
\SetSymbolFont{uprightglyphs}{boldsansup}{T1}{\savesffamily}{\savesfbfseries}{n}
\DeclareSymbolFont{italicglyphs} {T1}{\savermfamily}{\savermmdseries}{it}
\SetSymbolFont{italicglyphs} {normal}    {T1}{\savermfamily}{\savermmdseries}{it}
\SetSymbolFont{italicglyphs} {normalup}  {T1}{\savermfamily}{\savermmdseries}{n}
\SetSymbolFont{italicglyphs} {bold}      {T1}{\savermfamily}{\savermbfseries}{it}
\SetSymbolFont{italicglyphs} {boldup}    {T1}{\savermfamily}{\savermbfseries}{n}
\SetSymbolFont{italicglyphs} {sans}      {T1}{\savesffamily}{\savesfmdseries}{it}
\SetSymbolFont{italicglyphs} {sansup}    {T1}{\savesffamily}{\savesfmdseries}{n}
\SetSymbolFont{italicglyphs} {boldsans}  {T1}{\savesffamily}{\savesfbfseries}{it}
\SetSymbolFont{italicglyphs} {boldsansup}{T1}{\savesffamily}{\savesfbfseries}{n}

% Syntax of \DeclareMathSymobl:
% \DeclareMathSymbol {<symbol>} {<type>} {<sym-font>} {<slot>}
% Type              Meaning	            Example
% 0 or \mathord     Ordinary             $\alpha$
% 1 or \mathop      Large operator       $\sum$
% 2 or \mathbin     Binary operation     $\times$
% 3 or \mathrel     Relation             $\leq$
% 4 or \mathopen    Opening              $\langle$
% 5 or \mathclose   Closing              $\rangle$
% 6 or \mathpunct   Punctuation          ;
% 7 or \mathalpha   Alphabet character   A
% Example declaration:
% \DeclareMathSymbol{b}{0}{letters}{`b}

% Digits
\DeclareMathSymbol{0}{\mathalpha}{uprightglyphs}{`0}
\DeclareMathSymbol{1}{\mathalpha}{uprightglyphs}{`1}
\DeclareMathSymbol{2}{\mathalpha}{uprightglyphs}{`2}
\DeclareMathSymbol{3}{\mathalpha}{uprightglyphs}{`3}
\DeclareMathSymbol{4}{\mathalpha}{uprightglyphs}{`4}
\DeclareMathSymbol{5}{\mathalpha}{uprightglyphs}{`5}
\DeclareMathSymbol{6}{\mathalpha}{uprightglyphs}{`6}
\DeclareMathSymbol{7}{\mathalpha}{uprightglyphs}{`7}
\DeclareMathSymbol{8}{\mathalpha}{uprightglyphs}{`8}
\DeclareMathSymbol{9}{\mathalpha}{uprightglyphs}{`9}
% Operators and punctuation
%\DeclareMathSymbol{+}{\mathbin}  {operators}    {`+}
%\DeclareMathSymbol{+}{\mathbin}{symbols}{207}
	% From http://mirrors.ctan.org/fonts/newtx/tex/newtxmath.sty
% Not from uprightglyphs due to bad spacing
%\DeclareMathSymbol{=}{\mathrel}  {operators}    {`=}
% Not from uprightglyphs due to bad spacing
\DeclareMathSymbol{-}{\mathbin}{symbols}{0}
\DeclareMathSymbol{\leq}{\mathrel}{symbols}{20}
%   \let\le=\leq
\DeclareMathSymbol{\geq}{\mathrel}{symbols}{21}
%   \let\ge=\geq
	% From http://mirrors.ctan.org/fonts/newtx/tex/newtxmath.sty
\DeclareMathSymbol{.}{\mathord}  {uprightglyphs}{`.}
\DeclareMathSymbol{,}{\mathpunct}{uprightglyphs}{`,}
\DeclareMathSymbol{:}{\mathrel}  {uprightglyphs}{`:}
\let\colon\relax
\DeclareMathSymbol{\colon}{\mathpunct}{uprightglyphs}{`;}
\DeclareMathSymbol{;}{\mathpunct}{uprightglyphs}{`;}
\DeclareMathSymbol{/}{\mathord}  {uprightglyphs}{`/}
%\DeclareMathSymbol{/}{\mathop}   {uprightglyphs}{`/}
%	% This would icrease the spacing around the division slash slightly
\DeclareMathSymbol{!}{\mathord}  {uprightglyphs}{`!}
\DeclareMathSymbol{\mathdollar}{\mathord}{uprightglyphs}{`\$}
\DeclareRobustCommand{\$}{\ifmmode\mathdollar\else\symbol{`\$}\fi}
\DeclareMathSymbol{\mathpercent}{\mathord}{uprightglyphs}{`\%}
\DeclareRobustCommand{\%}{\ifmmode\mathpercent\else\symbol{`\%}\fi}
\DeclareMathSymbol{&}{\mathbin}{uprightglyphs}{`&}
%\DeclareMathSymbol{(}{\mathopen} {uprightglyphs}{`(}
%\DeclareMathSymbol{)}{\mathclose}{uprightglyphs}{`)}
%\DeclareMathSymbol{[}{\mathopen} {uprightglyphs}{`[}
%\DeclareMathSymbol{]}{\mathclose}{uprightglyphs}{`]}
%\DeclareMathSymbol{\prime}{\mathord}{extrasymbols}{"30}
% Use \prime from mathdesign-charter because it looks better than the one in kpfonts
\DeclareMathDelimiter{(}      {\mathopen} {uprightglyphs}{`(} {largesymbols}{"00}
\DeclareMathDelimiter{)}      {\mathclose}{uprightglyphs}{`)} {largesymbols}{"01}
\DeclareMathDelimiter{[}      {\mathopen} {uprightglyphs}{`[} {largesymbols}{"02}
\DeclareMathDelimiter{]}      {\mathclose}{uprightglyphs}{`]} {largesymbols}{"03}
\DeclareMathDelimiter{\lbrace}{\mathopen} {uprightglyphs}{`\{}{largesymbols}{"08}
\DeclareMathDelimiter{\rbrace}{\mathclose}{uprightglyphs}{`\}}{largesymbols}{"09}
% Uppercase Latin characters
\DeclareMathSymbol{A}{\mathalpha}{italicglyphs}{`A}
\DeclareMathSymbol{B}{\mathalpha}{italicglyphs}{`B}
\DeclareMathSymbol{C}{\mathalpha}{italicglyphs}{`C}
\DeclareMathSymbol{D}{\mathalpha}{italicglyphs}{`D}
\DeclareMathSymbol{E}{\mathalpha}{italicglyphs}{`E}
\DeclareMathSymbol{F}{\mathalpha}{italicglyphs}{`F}
\DeclareMathSymbol{G}{\mathalpha}{italicglyphs}{`G}
\DeclareMathSymbol{H}{\mathalpha}{italicglyphs}{`H}
\DeclareMathSymbol{I}{\mathalpha}{italicglyphs}{`I}
\DeclareMathSymbol{J}{\mathalpha}{italicglyphs}{`J}
\DeclareMathSymbol{K}{\mathalpha}{italicglyphs}{`K}
\DeclareMathSymbol{L}{\mathalpha}{italicglyphs}{`L}
\DeclareMathSymbol{M}{\mathalpha}{italicglyphs}{`M}
\DeclareMathSymbol{N}{\mathalpha}{italicglyphs}{`N}
\DeclareMathSymbol{O}{\mathalpha}{italicglyphs}{`O}
\DeclareMathSymbol{P}{\mathalpha}{italicglyphs}{`P}
\DeclareMathSymbol{Q}{\mathalpha}{italicglyphs}{`Q}
\DeclareMathSymbol{R}{\mathalpha}{italicglyphs}{`R}
\DeclareMathSymbol{S}{\mathalpha}{italicglyphs}{`S}
\DeclareMathSymbol{T}{\mathalpha}{italicglyphs}{`T}
\DeclareMathSymbol{U}{\mathalpha}{italicglyphs}{`U}
\DeclareMathSymbol{V}{\mathalpha}{italicglyphs}{`V}
\DeclareMathSymbol{W}{\mathalpha}{italicglyphs}{`W}
\DeclareMathSymbol{X}{\mathalpha}{italicglyphs}{`X}
\DeclareMathSymbol{Y}{\mathalpha}{italicglyphs}{`Y}
\DeclareMathSymbol{Z}{\mathalpha}{italicglyphs}{`Z}
% lowercase Latin characters
\DeclareMathSymbol{a}{\mathalpha}{italicglyphs}{`a}
\DeclareMathSymbol{b}{\mathalpha}{italicglyphs}{`b}
\DeclareMathSymbol{c}{\mathalpha}{italicglyphs}{`c}
\DeclareMathSymbol{d}{\mathalpha}{italicglyphs}{`d}
\DeclareMathSymbol{e}{\mathalpha}{italicglyphs}{`e}
\DeclareMathSymbol{f}{\mathalpha}{italicglyphs}{`f}
\DeclareMathSymbol{g}{\mathalpha}{italicglyphs}{`g}
\DeclareMathSymbol{h}{\mathalpha}{italicglyphs}{`h}
\DeclareMathSymbol{i}{\mathalpha}{italicglyphs}{`i}
\DeclareMathSymbol{\imath}{\mathalpha}{italicglyphs}{"19}
\DeclareMathSymbol{j}{\mathalpha}{italicglyphs}{`j}
\DeclareMathSymbol{\jmath}{\mathalpha}{italicglyphs}{"1A}
\DeclareMathSymbol{k}{\mathalpha}{italicglyphs}{`k}
\DeclareMathSymbol{l}{\mathalpha}{italicglyphs}{`l}
\DeclareMathSymbol{m}{\mathalpha}{italicglyphs}{`m}
\DeclareMathSymbol{n}{\mathalpha}{italicglyphs}{`n}
\DeclareMathSymbol{o}{\mathalpha}{italicglyphs}{`o}
\DeclareMathSymbol{p}{\mathalpha}{italicglyphs}{`p}
\DeclareMathSymbol{q}{\mathalpha}{italicglyphs}{`q}
\DeclareMathSymbol{r}{\mathalpha}{italicglyphs}{`r}
\DeclareMathSymbol{s}{\mathalpha}{italicglyphs}{`s}
\DeclareMathSymbol{t}{\mathalpha}{italicglyphs}{`t}
\DeclareMathSymbol{u}{\mathalpha}{italicglyphs}{`u}
\DeclareMathSymbol{v}{\mathalpha}{italicglyphs}{`v}
\DeclareMathSymbol{w}{\mathalpha}{italicglyphs}{`w}
\DeclareMathSymbol{x}{\mathalpha}{italicglyphs}{`x}
\DeclareMathSymbol{y}{\mathalpha}{italicglyphs}{`y}
\DeclareMathSymbol{z}{\mathalpha}{italicglyphs}{`z}

% Redefine \cdots so that its appearance matches \ldots, \ddots, and \vdots:
%%% Use math italic, not text, version of dot, in \vdots and \ddots definitions
\makeatletter
\def\cdots{\mathinner{\mkern1mu\raise2.5\p@
    \vbox{\kern7\p@\hbox{$\m@th.$}}\mkern4mu
    \raise2.5\p@\hbox{$\m@th.$}\mkern4mu\raise2.5\p@\hbox{$\m@th.$}\mkern1mu}}
    % \raise2.5\p@ instead of \raise4\p@ to match \cdot
    % \mkern4mu  instead of \mkern2mu  to match \ldots
% Inspired by:
% \def\ddots{\mathinner{\mkern1mu\raise7\p@
%     \vbox{\kern7\p@\hbox{$\m@th.$}}\mkern2mu
%     \raise4\p@\hbox{$\m@th.$}\mkern2mu\raise\p@\hbox{$\m@th.$}\mkern1mu}}
\makeatother
	% Based on http://mirrors.ctan.org/fonts/newtx/tex/newtxmath.sty
%% Sansserif Greek letters
%\DeclareSymbolFont{lgrgreek}{LGR}{\savesffamily}{\savesfmdseries}{it}
%\SetSymbolFont{lgrgreek}{sans}    {LGR}{\savesffamily}{\savesfmdseries}{it}
%\SetSymbolFont{lgrgreek}{boldsans}{LGR}{\savesffamily}{\savesfbfseries}{it}

% The following is taken from
% https://tex.stackexchange.com/questions/116389/automatic-upright-math-when-text-is-in-italic/116399#116399
% Filling in ``missing'' Greek glyphs for completeness
% (not really necessary, since they look identical to Latin glyphs and are thus almost never used)
% ==>
\newcommand{\omicron}{o}
\newcommand{\Digamma}{F}
\newcommand{\Alpha}  {A}
\newcommand{\Beta}   {B}
\newcommand{\Epsilon}{E}
\newcommand{\Zeta}   {Z}
\newcommand{\Eta}    {H}
\newcommand{\Iota}   {I}
\newcommand{\Kappa}  {K}
\newcommand{\Mu}     {M}
\newcommand{\Nu}     {N}
\newcommand{\Omicron}{O}
\newcommand{\Rho}    {P}
\newcommand{\Tau}    {T}
\newcommand{\Chi}    {X}
\newcommand{\omicronup}{\mathup{o}}
\newcommand{\Digammaup}{\mathup{F}}
\newcommand{\Alphaup}  {\mathup{A}}
\newcommand{\Betaup}   {\mathup{B}}
\newcommand{\Epsilonup}{\mathup{E}}
\newcommand{\Zetaup}   {\mathup{Z}}
\newcommand{\Etaup}    {\mathup{H}}
\newcommand{\Iotaup}   {\mathup{I}}
\newcommand{\Kappaup}  {\mathup{K}}
\newcommand{\Muup}     {\mathup{M}}
\newcommand{\Nuup}     {\mathup{N}}
\newcommand{\Omicronup}{\mathup{O}}
\newcommand{\Rhoup}    {\mathup{P}}
\newcommand{\Tauup}    {\mathup{T}}
\newcommand{\Chiup}    {\mathup{X}}
% <==

% Save original definitions of the Greek letters
% ==>
\makeatletter
\@for\@tempa:=%
	alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,lambda,mu,nu,xi,%
	omicron,pi,rho,sigma,varsigma,tau,upsilon,phi,chi,psi,omega,digamma,%
	Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
	Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
\do{%
	\expandafter\let\csname\@tempa orig\expandafter\endcsname\csname\@tempa\endcsname%
	\expandafter\let\csname\@tempa uporig\expandafter\endcsname\csname\@tempa up\endcsname%
}%
\makeatother
% <==

% LGR-encoded Greek letters
% ==>
\newcommand{\textformath}[1]{%
	\IfInBoldMode%
	\IfInUpMode\textbf{#1}\else\textit{\bfseries #1}\fi\relax%
	\else
	\IfInUpMode\textup{#1}\else\textit{#1}\fi\relax%
	\fi\relax%
}
% The double curly braces in this section are necessary to be able to use Greek letters
% in subscripts and superscripts without having to enclose theme in curly braces;
% for example, $\sigma_\epsilon$ instead of $\sigma_{\epsilon}$.
% Uppercase
\newcommand{\AlphaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont A}}}}
\newcommand{\BetaLGR}    {{\mathord{\textformath{\fontencoding{LGR}\selectfont B}}}}
\newcommand{\GammaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont G}}}}
\newcommand{\DeltaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont D}}}}
\newcommand{\EpsilonLGR} {{\mathord{\textformath{\fontencoding{LGR}\selectfont E}}}}
\newcommand{\ZetaLGR}    {{\mathord{\textformath{\fontencoding{LGR}\selectfont Z}}}}
\newcommand{\EtaLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont H}}}}
\newcommand{\ThetaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont J}}}}
\newcommand{\IotaLGR}    {{\mathord{\textformath{\fontencoding{LGR}\selectfont I}}}}
\newcommand{\KappaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont K}}}}
\newcommand{\LambdaLGR}  {{\mathord{\textformath{\fontencoding{LGR}\selectfont L}}}}
\newcommand{\MuLGR}      {{\mathord{\textformath{\fontencoding{LGR}\selectfont M}}}}
\newcommand{\NuLGR}      {{\mathord{\textformath{\fontencoding{LGR}\selectfont N}}}}
\newcommand{\XiLGR}      {{\mathord{\textformath{\fontencoding{LGR}\selectfont X}}}}
\newcommand{\OmicronLGR} {{\mathord{\textformath{\fontencoding{LGR}\selectfont O}}}}
\newcommand{\PiLGR}      {{\mathord{\textformath{\fontencoding{LGR}\selectfont P}}}}
\newcommand{\RhoLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont R}}}}
\newcommand{\SigmaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont S}}}}
\newcommand{\TauLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont T}}}}
\newcommand{\UpsilonLGR} {{\mathord{\textformath{\fontencoding{LGR}\selectfont U}}}}
\newcommand{\PhiLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont F}}}}
\newcommand{\ChiLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont Q}}}}
\newcommand{\PsiLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont Y}}}}
\newcommand{\OmegaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont W}}}}
\newcommand{\DigammaLGR} {{\mathord{\textformath{\fontencoding{LGR}\selectfont \char195}}}}
% lowercase
\newcommand{\alphaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont a}}}}
\newcommand{\betaLGR}    {{\mathord{\textformath{\fontencoding{LGR}\selectfont b}}}}
\newcommand{\gammaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont g}}}}
\newcommand{\deltaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont d}}}}
\newcommand{\epsilonLGR} {{\mathord{\textformath{\fontencoding{LGR}\selectfont e}}}}
\newcommand{\zetaLGR}    {{\mathord{\textformath{\fontencoding{LGR}\selectfont z}}}}
\newcommand{\etaLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont h}}}}
\newcommand{\thetaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont j}}}}
\newcommand{\iotaLGR}    {{\mathord{\textformath{\fontencoding{LGR}\selectfont i}}}}
\newcommand{\kappaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont k}}}}
\newcommand{\lambdaLGR}  {{\mathord{\textformath{\fontencoding{LGR}\selectfont l}}}}
\newcommand{\muLGR}      {{\mathord{\textformath{\fontencoding{LGR}\selectfont m}}}}
\newcommand{\nuLGR}      {{\mathord{\textformath{\fontencoding{LGR}\selectfont n}}}}
\newcommand{\xiLGR}      {{\mathord{\textformath{\fontencoding{LGR}\selectfont x}}}}
\newcommand{\omicronLGR} {{\mathord{\textformath{\fontencoding{LGR}\selectfont o}}}}
\newcommand{\piLGR}      {{\mathord{\textformath{\fontencoding{LGR}\selectfont p}}}}
\newcommand{\rhoLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont r}}}}
\newcommand{\sigmaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont s\noboundary}}}}
% \noboundary prevents sigma from being replaced by the word-end sigma (varsigma),
% see http://mirrors.ctan.org/macros/latex/contrib/textgreek/textgreek.pdf
\newcommand{\varsigmaLGR}{{\mathord{\textformath{\fontencoding{LGR}\selectfont c}}}}
\newcommand{\tauLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont t}}}}
\newcommand{\upsilonLGR} {{\mathord{\textformath{\fontencoding{LGR}\selectfont u}}}}
\newcommand{\phiLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont f}}}}
\newcommand{\chiLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont q}}}}
\newcommand{\psiLGR}     {{\mathord{\textformath{\fontencoding{LGR}\selectfont y}}}}
\newcommand{\omegaLGR}   {{\mathord{\textformath{\fontencoding{LGR}\selectfont w}}}}
\newcommand{\digammaLGR} {{\mathord{\textformath{\fontencoding{LGR}\selectfont \char147}}}}
% Uppercase, upright
\newcommand{\AlphaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont A}}}}
\newcommand{\BetaupLGR}    {{\mathord{\textup{\fontencoding{LGR}\selectfont B}}}}
\newcommand{\GammaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont G}}}}
\newcommand{\DeltaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont D}}}}
\newcommand{\EpsilonupLGR} {{\mathord{\textup{\fontencoding{LGR}\selectfont E}}}}
\newcommand{\ZetaupLGR}    {{\mathord{\textup{\fontencoding{LGR}\selectfont Z}}}}
\newcommand{\EtaupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont H}}}}
\newcommand{\ThetaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont J}}}}
\newcommand{\IotaupLGR}    {{\mathord{\textup{\fontencoding{LGR}\selectfont I}}}}
\newcommand{\KappaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont K}}}}
\newcommand{\LambdaupLGR}  {{\mathord{\textup{\fontencoding{LGR}\selectfont L}}}}
\newcommand{\MuupLGR}      {{\mathord{\textup{\fontencoding{LGR}\selectfont M}}}}
\newcommand{\NuupLGR}      {{\mathord{\textup{\fontencoding{LGR}\selectfont N}}}}
\newcommand{\XiupLGR}      {{\mathord{\textup{\fontencoding{LGR}\selectfont X}}}}
\newcommand{\OmicronupLGR} {{\mathord{\textup{\fontencoding{LGR}\selectfont O}}}}
\newcommand{\PiupLGR}      {{\mathord{\textup{\fontencoding{LGR}\selectfont P}}}}
\newcommand{\RhoupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont R}}}}
\newcommand{\SigmaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont S}}}}
\newcommand{\TauupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont T}}}}
\newcommand{\UpsilonupLGR} {{\mathord{\textup{\fontencoding{LGR}\selectfont U}}}}
\newcommand{\PhiupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont F}}}}
\newcommand{\ChiupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont Q}}}}
\newcommand{\PsiupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont Y}}}}
\newcommand{\OmegaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont W}}}}
\newcommand{\DigammaupLGR} {{\mathord{\textup{\fontencoding{LGR}\selectfont \char195}}}}
% lowercase, upright
\newcommand{\alphaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont a}}}}
\newcommand{\betaupLGR}    {{\mathord{\textup{\fontencoding{LGR}\selectfont b}}}}
\newcommand{\gammaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont g}}}}
\newcommand{\deltaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont d}}}}
\newcommand{\epsilonupLGR} {{\mathord{\textup{\fontencoding{LGR}\selectfont e}}}}
\newcommand{\zetaupLGR}    {{\mathord{\textup{\fontencoding{LGR}\selectfont z}}}}
\newcommand{\etaupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont h}}}}
\newcommand{\thetaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont j}}}}
\newcommand{\iotaupLGR}    {{\mathord{\textup{\fontencoding{LGR}\selectfont i}}}}
\newcommand{\kappaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont k}}}}
\newcommand{\lambdaupLGR}  {{\mathord{\textup{\fontencoding{LGR}\selectfont l}}}}
\newcommand{\muupLGR}      {{\mathord{\textup{\fontencoding{LGR}\selectfont m}}}}
\newcommand{\nuupLGR}      {{\mathord{\textup{\fontencoding{LGR}\selectfont n}}}}
\newcommand{\xiupLGR}      {{\mathord{\textup{\fontencoding{LGR}\selectfont x}}}}
\newcommand{\omicronupLGR} {{\mathord{\textup{\fontencoding{LGR}\selectfont o}}}}
\newcommand{\piupLGR}      {{\mathord{\textup{\fontencoding{LGR}\selectfont p}}}}
\newcommand{\rhoupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont r}}}}
\newcommand{\sigmaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont s\noboundary}}}}
% \noboundary prevents sigma from being replaced by the word-end sigma (varsigma),
% see http://mirrors.ctan.org/macros/latex/contrib/textgreek/textgreek.pdf
\newcommand{\varsigmaupLGR}{{\mathord{\textup{\fontencoding{LGR}\selectfont c}}}}
\newcommand{\tauupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont t}}}}
\newcommand{\upsilonupLGR} {{\mathord{\textup{\fontencoding{LGR}\selectfont u}}}}
\newcommand{\phiupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont f}}}}
\newcommand{\chiupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont q}}}}
\newcommand{\psiupLGR}     {{\mathord{\textup{\fontencoding{LGR}\selectfont y}}}}
\newcommand{\omegaupLGR}   {{\mathord{\textup{\fontencoding{LGR}\selectfont w}}}}
\newcommand{\digammaupLGR} {{\mathord{\textup{\fontencoding{LGR}\selectfont \char147}}}}
% <==

% Based on description of the TS1 encoding in
% http://ctan.math.illinois.edu/macros/latex/doc/encguide.pdf:
%\let \oldpm    \pm
%\let \oldtimes \times
%\let \olddiv   \div
%\makeatletter
%\newcommand{\pmsf}   {\mathbin{\text{\usefont{TS1}{\sfdefault}{\f@series}{n}\char"B1}}}
%\newcommand{\timessf}{\mathbin{\text{\usefont{TS1}{\sfdefault}{\f@series}{n}\char"D6}}}
%\newcommand{\divsf}  {\mathbin{\text{\usefont{TS1}{\sfdefault}{\f@series}{n}\char"F6}}}
%\makeatother

% Use LGR-encoded Greek letters for \mathversion{sans}
% ==>
\makeatletter

% Save original definition of \varepsilon etc.
\@for\@tempa:=%
	epsilon,theta,pi,rho,phi%
\do{%
	\expandafter\let\csname var\@tempa orig\expandafter\endcsname\csname var\@tempa\endcsname%
}

\newcommand*{\sansmath}{%
	\@for\@tempa:=%
	alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,lambda,mu,nu,xi,%
	omicron,pi,rho,sigma,varsigma,tau,upsilon,phi,chi,psi,omega,digamma,%
	Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
	Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
	\do{%
		\expandafter\let\csname\@tempa\expandafter\endcsname\csname\@tempa LGR\endcsname%
		\expandafter\let\csname\@tempa up\expandafter\endcsname\csname\@tempa upLGR\endcsname%
		\expandafter\let\csname up\@tempa\expandafter\endcsname\csname\@tempa upLGR\endcsname%
	}%
	\@for\@tempa:=%
		epsilon,theta,pi,rho,phi%
	\do{%
		\expandafter\let\csname var\@tempa\expandafter\endcsname\csname\@tempa\endcsname%
	}%
	%\renewcommand{\pm}{\pmsf}%
	%\renewcommand{\times}{\timessf}%
	%\renewcommand{\div}{\divsf}%
}
% <==

% Switch back to the original Greek letters for \mathversion{normal}, i.e., the serif font
% ==>
\newcommand*{\unsansmath}{%
	\@for\@tempa:=%
	alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,lambda,mu,nu,xi,%
	omicron,pi,rho,sigma,varsigma,tau,upsilon,phi,chi,psi,omega,digamma,%
	Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
	Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
	\do{%
		\expandafter\let\csname\@tempa\expandafter\endcsname\csname\@tempa orig\endcsname%
		\expandafter\let\csname\@tempa up\expandafter\endcsname\csname\@tempa uporig\endcsname%
		\expandafter\let\csname up\@tempa\expandafter\endcsname\csname\@tempa uporig\endcsname%
	}%
	\@for\@tempa:=%
		epsilon,theta,pi,rho,phi%
	\do{%
		\expandafter\let\csname var\@tempa\expandafter\endcsname\csname var\@tempa orig\endcsname%
	}%
	%\renewcommand{\pm}{\oldpm}%
	%\renewcommand{\times}{\oldtimes}%
	%\renewcommand{\div}{\olddiv}%
}
% <==

%% If you would like to use LGR-encoded Greek letters also for the serif font
%% ==>
%\renewcommand*{\unsansmath}{%
%	\@for\@tempa:=%
%		alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,lambda,mu,nu,xi,%
%		omicron,pi,rho,sigma,varsigma,tau,upsilon,phi,chi,psi,omega,digamma,%
%		Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
%		Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
%		\do{%
%			\expandafter\let\csname\@tempa\expandafter\endcsname\csname\@tempa LGR\endcsname%
%			\expandafter\let\csname\@tempa up\expandafter\endcsname\csname\@tempa upLGR\endcsname%
%			\expandafter\let\csname up\@tempa\expandafter\endcsname\csname\@tempa upLGR\endcsname%
%		}%
%	%\renewcommand{\pm}{\pmsf}%
%	%\renewcommand{\times}{\timessf}%
%	%\renewcommand{\div}{\divsf}%
%}
%% <==

\newcommand*{\upgreekletters}{%
	\@for\@tempa:=%
	alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,lambda,mu,nu,xi,%
	omicron,pi,rho,sigma,varsigma,tau,upsilon,phi,chi,psi,omega,digamma,%
	Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
	Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
	\do{%
		\expandafter\let\csname\@tempa\expandafter\endcsname\csname\@tempa up\endcsname%
	}%
}
\newcommand*{\itgreekletters}{%
	\@for\@tempa:=%
	alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,lambda,mu,nu,xi,%
	omicron,pi,rho,sigma,varsigma,tau,upsilon,phi,chi,psi,omega,digamma,%
	Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Iota,Kappa,Lambda,Mu,Nu,Xi,%
	Omicron,Pi,Rho,Sigma,Tau,Upsilon,Phi,Chi,Psi,Omega,Digamma%
	\do{%
		\expandafter\let\csname\@tempa\expandafter\endcsname\csname\@tempa orig\endcsname%
	}%
}

\makeatother

%\makeatletter
%	\@for\@tempa:=%
%	%alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,lambda,mu,nu,xi,%
%	%pi,rho,sigma,varsigma,tau,upsilon,phi,chi,psi,omega,digamma,%
%	Gamma,Delta,Theta,Lambda,Xi,Pi,Sigma,Upsilon,Phi,Psi,Omega%
%	\do{\expandafter\let\csname\@tempa\expandafter\endcsname\csname other\@tempa\endcsname}%
%\makeatother

% Fix the \bm command so that it also works properly in the sans mathversions
% ==>
\let \bmorig \bm
\renewcommand{\bm}[1]{%
	\IfInSansMode%
		\textbf{\mathversion{boldsans}\(#1\)}%
	\else%
		{\InBoldModetrue\bmorig{#1}}%
	\fi\relax%
}
% <==
\renewcommand{\mathbf}[1]{\bm{#1}}
\renewcommand{\boldsymbol}[1]{\bm{#1}}
\newcommand{\mathbfit}[1]{\bm{#1}}
%\renewcommand{\mathcal}[1]{\mathscr{#1}}
\renewcommand{\mathscr}[1]{\mathcal{#1}}

% Apply sansmath etc. automagically
% ==>
\newif\IfInSansMode
\newif\IfInBoldMode
\newif\IfInUpMode
\let \oldsf \sffamily
\renewcommand*{\sffamily}{%
	\oldsf\sansmath\InSansModetrue%
	\IfInBoldMode\mathversion{boldsans}\else\mathversion{sans}\fi\relax%
}
\let \oldbf \bfseries
\renewcommand*{\bfseries}{%
	\oldbf\InBoldModetrue%
	\IfInSansMode\sansmath\mathversion{boldsans}\else\mathversion{bold}\fi\relax%
}
\let \oldmd \mdseries
\renewcommand*{\mdseries}{%
	\oldmd\InBoldModefalse%
	\IfInSansMode\sansmath\mathversion{sans}\else\mathversion{normal}\fi\relax%
}
\let \oldnorm \normalfont
\renewcommand*{\normalfont}{%
	\oldnorm\InSansModefalse\InBoldModefalse\mathversion{normal}%
	\unsansmath%
}
\let \oldrm \rmfamily
\renewcommand*{\rmfamily}{%
	\oldrm\InSansModefalse%
	\IfInBoldMode\mathversion{bold}\else\mathversion{normal}\fi\relax%
	\unsansmath%
}
% <==

% Make \mathnormal obey the currently active \mathversion ==>
\let \mathnormalorig \mathnormal
\renewcommand{\mathnormal}[1]{%
	\IfInSansMode%
		\IfInBoldMode%
			\mathversion{boldsans}%
			{\textbf{\(#1\)}}%
		\else%
			\mathversion{sans}%
			{\textmd{\(#1\)}}%
		\fi\relax%	
	\else%
		\mathnormalorig{#1}%
	\fi\relax%
}
% <==

% Adjust \mathrm to the curretly active \mathversion.
% We set it up such that also in sansserif mode, \mathrm activates the serif font.
% ==>
%\DeclareMathAlphabet{\mathrm}{OT1}{\savermfamily}{\savermmdseries}{n}
\let \mathrmorig \mathrm
\renewcommand{\mathrm}[1]{%
	\IfInSansMode%
		{\textrm{%
			\IfInBoldMode%
				\mathversion{bold}%
				\(\mathrmorig{#1}\)%
			\else%
				\mathversion{normal}%
				\(\mathrmorig{#1}\)%
			\fi\relax%
		}}%
	\else%
		\mathrmorig{#1}%
	\fi\relax%
}
% <==

% Define \mathup to activate \upshape without switching to the serif font
% (in contrast to \mathrm)
% ==>
\newcommand{\mathup}[1]{%
	\IfInSansMode%
		{\textup{%
			\InUpModetrue%
				\IfInBoldMode%
				\mathversion{boldsansup}%
				\(#1\)%
			\else%
				\mathversion{sansup}%
				\(#1\)%
			\fi\relax%
		}}%
	\else%
		{\upgreekletters\mathrm{#1}\itgreekletters}%
	\fi\relax%
}
\newcommand{\mathbfup}[1]{%
	\mathbf{\mathup{#1}}
}
% <==

% If you would like to redefine \mathup also for the serif font:
% ==>
\renewcommand{\mathup}[1]{%
	\IfInSansMode%
		{\textup{%
			\InUpModetrue%
			\IfInBoldMode%
				\mathversion{boldsansup}%
				\(#1\)%
			\else%
				\mathversion{sansup}%
				\(#1\)%
			\fi\relax%
		}}%
	\else%
		{\textup{%
			\InUpModetrue%
			\upgreekletters%
			\IfInBoldMode%
				\mathversion{boldup}%
				\(#1\)%
			\else%
				\mathversion{normalup}%
				\(#1\)%
			\fi\relax%
		}}%
	\fi\relax%
}
\renewcommand{\mathbfup}[1]{{%
	\InBoldModetrue%
	\IfInSansMode%
		{\mathbf{\mathup{#1}}}%
	\else%
		{\upgreekletters\mathbf{\mathup{#1}}\itgreekletters}%
	\fi\relax%
}}
% <==

%\SetMathAlphabet{\mathrm}{normal}{OT1}{\savermfamily}{\savermmdseries}{n}
%\DeclareMathAlphabet{\mathrm}{OT1}{\savermfamily}{\savermmdseries}{n}
\renewcommand{\mathrm}[1]{%
	{\textup{%
		\protect\InUpModetrue%
		\IfInBoldMode%
			\mathversion{boldup}%
			\protect\upgreekletters%
			\(#1\)%
		\else%
			\mathversion{normalup}%
			\protect\upgreekletters%
			\(#1\)%
		\fi\relax%
	 }}%
}

% Make the LaTeX-defined operators obey sansserif math
% ==>
\let \operatornameorig \operatorname
\renewcommand{\operatorname}[1]{%
	\operatornameorig{\mathup{#1}}%
}
\makeatletter
\@for\@tempa:=%
	arccos,arccot,arccsc,arcsec,arcsin,arctan,arg,cos,cosh,cot,coth,csc,%
	deg,det,dim,exp,gcd,hom,inf,ker,lg,lim,liminf,limsup,ln,log,max,min,%
	Pr,sec,sin,sinh,sup,tan,tanh%
\do{%
	\expandafter\let\csname\@tempa\endcsname\relax%
}%
\makeatother
\DeclareMathOperator {\arccos}{\mathup{arccos}}
\DeclareMathOperator {\arccot}{\mathup{arccot}}
\DeclareMathOperator {\arccsc}{\mathup{arccsc}}
\DeclareMathOperator {\arcsec}{\mathup{arcsec}}
\DeclareMathOperator {\arcsin}{\mathup{arcsin}}
\DeclareMathOperator {\arctan}{\mathup{arctan}}
\DeclareMathOperator {\arg}   {\mathup{arg}}
\DeclareMathOperator {\cos}   {\mathup{cos}}
\DeclareMathOperator {\cosh}  {\mathup{cosh}}
\DeclareMathOperator {\cot}   {\mathup{cot}}
\DeclareMathOperator {\coth}  {\mathup{coth}}
\DeclareMathOperator {\csc}   {\mathup{csc}}
\DeclareMathOperator {\deg}   {\mathup{deg}}
\DeclareMathOperator {\det}   {\mathup{det}}
\DeclareMathOperator {\dim}   {\mathup{dim}}
\DeclareMathOperator {\exp}   {\mathup{exp}}
\DeclareMathOperator {\gcd}   {\mathup{gcd}}
\DeclareMathOperator*{\hom}   {\mathup{hom}}
\DeclareMathOperator*{\inf}   {\mathup{inf}}
\DeclareMathOperator {\ker}   {\mathup{ker}}
\DeclareMathOperator {\lg}    {\mathup{lg}}
\DeclareMathOperator {\lim}   {\mathup{lim}}
\DeclareMathOperator*{\liminf}{\mathup{lim\,inf}}
\DeclareMathOperator*{\limsup}{\mathup{lim\,sup}}
\DeclareMathOperator {\ln}    {\mathup{ln}}
\DeclareMathOperator {\log}   {\mathup{log}}
\DeclareMathOperator*{\max}   {\mathup{max}}
\DeclareMathOperator*{\min}   {\mathup{min}}
\DeclareMathOperator {\Pr}    {\mathup{Pr}}
\DeclareMathOperator {\sec}   {\mathup{sec}}
\DeclareMathOperator {\sin}   {\mathup{sin}}
\DeclareMathOperator {\sinh}  {\mathup{sinh}}
\DeclareMathOperator*{\sup}   {\mathup{sup}}
\DeclareMathOperator {\tan}   {\mathup{tan}}
\DeclareMathOperator {\tanh}  {\mathup{tanh}}
% <==

